Breaking and (Partially) Fixing Provably Secure Onion Routing

After several years of research on onion routing, Camenisch and Lysyanskaya, in an attempt at rigorous analysis, defined an ideal functionality in the universal composability model, together with properties that protocols have to meet to achieve provable security. A whole family of systems based their security proofs on this work. However, analyzing HORNET and Sphinx, two instances from this family, we show that this proof strategy is broken. We discover a previously unknown vulnerability that breaks anonymity completely, and explain a known one. Both should not exist if privacy is proven correctly. In this work, we analyze and fix the proof strategy used for this family of systems. After proving the efficacy of the ideal functionality, we show how the original properties are flawed and suggest improved, effective properties in their place. Finally, we discover another common mistake in the proofs. We demonstrate how to avoid it by showing our improved properties for one protocol, thus partially fixing the family of provably secure onion routing protocols.

==> protocols/sphinxForwardCorrection.tex <==
Sphinx can be attacked by manipulation of the payload (through active adversaries) that is not detected by honest mix nodes. One way to circumvent this attack is to adapt the protocol in a way that modifications upon the payload done by active adversaries are detected and discarded by honest nodes.

This can be achieved by adapting the protocol to include the payload layers $\delta_i$ in the tag $\gamma_i$ during header creation.

\subsection{Creating a mix header}
It is used as a subroutine (denoted CreateHeader) for the procedure to create forward messages.

\emph{Input}: $(\Delta,I,\mathcal{P},\underline{\mathcal{Q}})$, a destination address $\Delta \in \mathcal{D}$, an identifier $I \in \{0,1\}^\kappa$, a
sequence of mix nodes $\mathcal{P} = \{n_0,n_1,\dots,n_{\nu - 1}\}$ with $\nu \leq r$ and $|\Delta| \leq (2(r-\nu)+1)\kappa$, \textbf{and a sequence of payload layers} $\underline{\mathcal{Q} = (\delta_0,\delta_1,\dots,\delta_{\nu-1})}$.

Pick a random $x \in_R \mathbb{Z}_q^*$.
Compute a sequence of $\nu$ tuples $(\alpha_0, \beta_0, \gamma_0) \dots (\alpha_{\nu - 1}, \beta_{\nu - 1}, \gamma_{\nu - 1})$.
\begin{itemize}
  \item $\alpha_0 = g^x, s_0 = y_{n_0}^x, b_0=h_b(\alpha_0,s_0)$
  \item $\alpha_1 = g^{xb_0}, s_1 = y_{n_1}^{xb_0}, b_1=h_b(\alpha_1,s_1)$
  \item $\ldots$
  \item $\alpha_{\nu -1} = g^{xb_0b_1\dots b_{\nu -2}}, s_{\nu -1} = y_{n_{\nu -1}}^{xb_0b_1\dots b_{\nu -2}}, b_{\nu -1}=h_b(\alpha_{\nu -1},s_{\nu -1})$
\end{itemize}

The $\alpha_i$ are the group elements, the $s_i$ are the Diffie-Hellman shared secrets, and the $b_i$ are the blinding factors.


Compute the filler strings $\phi_0,\ldots,\phi_{\nu -1}$:
Let $\phi_0 = \epsilon$ and
\(\phi_i = \{\phi_{i-1}||0_{2\kappa}\} \oplus \left\{ \rho(h_\rho(s_{i-1}))_{[(2(r-i)+3)\kappa .. (2r+3)\kappa - 1]} \right\}\)
with $|\phi_i| = 2i\kappa $.

Compute a sequence of mix headers $M_{\nu - 1},M_{\nu - 2}, \dots, M_0$ with
$M_i = (\alpha_i,\beta_i,\gamma_i) \in \mathcal{G}^* \times \{0,1\}^{(2r+1)\kappa} \times \{0,1\}^\kappa$.
Let \(\beta_{\nu -1} = \{\{\Delta || I || 0_{(2(r-\nu)+2)\kappa-|\Delta|}\} \oplus \{\rho(h_\rho(s_{\nu -1}))_{[0..(2(r-\nu)+3)\kappa -1]} \}\}||\phi_{\nu-1}\).

For $0 \leq i < \nu -1$:
\begin{itemize}
  \item $\beta_i = \left\{n_{i+1}||\gamma_{i+1}||\beta_{i+1_{[0..(2r-1)\kappa -1]}} \right\} \oplus \rho(h_\rho(s_i))_{[0..(2r+1)\kappa -1]}$
  \item $\gamma_i = \mu(h_\mu(s_i),\beta_i,\underline{\delta_i})$
\end{itemize}

\emph{Output}: the mix header $M_0$ and the sequence of shared secrets $s_0,\dots,s_{\nu -1}$.


==> protocols/sphinxOriginal.tex <==
The following sections regarding the notation and protocol description are taken from~\cite{danezis_sphinx:_2009}.

\subsection{Notation}


Let \(\kappa\) be a security parameter. Let $r$ be the maximum number of nodes that a
Sphinx mix message will traverse before being delivered to its destination. It is suggested to use \(r=5\).

Define the following:
$\mathcal{G}$: A prime-order cyclic group satisfying the Decisional Diffie-Hellman Assumption.
$\mathcal{G^*}$ is the set of non-identity elements of $\mathcal{G}$. The element $g$ is a generator of
\(\mathcal{G}\), and $q$ is the (prime) order of $\mathcal{G}$, with $q \approx 2^{2\kappa}$.

A number of hash functions, which we model by random oracles:
\begin{itemize}
  \item $h_\mu \from \mathcal{G^*} \to \{0,1\}^\kappa$, used to key $\mu$
  \item $h_\rho \from \mathcal{G^*} \to \{0,1\}^\kappa$, used to key $\rho$
  \item $h_\pi \from \mathcal{G^*} \to \{0,1\}^\kappa$, used to key $\pi$
  \item $h_\tau \from \mathcal{G^*} \to \{0,1\}^{2\kappa}$, used to identify previously seen elements of $\mathcal{G^*}$
  \item $h_b \from \mathcal{G^*} \times \mathcal{G^*} \to \mathbb{Z}_q^*$, used to compute blinding factors
\end{itemize}

These functions are implemented using appropriately truncated SHA256 hash functions.
\paragraph{MAC $\mu \from \{0,1\}^\kappa \times \{0,1\}^* \to \{0,1\}^\kappa$}
 is a message authentication code (MAC). In the proof
(section 4.2 in~\cite{danezis_sphinx:_2009}), $\mu$ needs to behave as a hash function even if the adversary gains
knowledge of the key. Therefore, this function to be modelled as a random oracle instead of a PRF. 
An implementation would use something like SHA256-HMAC-128.

\paragraph{PRG $\rho \from \{0,1\}^\kappa \to \{0,1\}^{(2r+3)\kappa}$}
is a pseudo-random generator (PRG) used to generate the keystream for a stream cipher. Similar to $\mu$,
it is modeled as a random oracle, instead of a PRG, as the adversary may learn the input to $\rho$.
An implementation may use any secure stream cipher or block cipher in counter mode.

\paragraph{PRP $\pi \from \{0,1\}^\kappa \times \{0,1\}^{l_\pi}$}
is a family of pseudo random permutations (PRPs). $l_\pi$ is the size of the payload that can be transmitted
s message over Sphinx using a single packet (plus $\kappa$ bits of overhead). $\pi^{-1}$ is keyed the inverse PRP
of \(\pi\), both are easy to compute given key $k$.
An implementation may use the LIONESS PRP to implement \(\pi\).

Each mix node has an identifier $n \in \mathcal{N}$, private key $x_n \in_R \mathbb{Z}_q^*$ and public key $y_n = g^{x_n} \in \mathcal{G}^*$.
All pairs $(n,y_n)$ are published in an authentic way.
$\mathcal{D} \subset \{0,1\}^{\leq 2r\kappa}$ is a set of destination addresses (may be email addresses).
$\mathcal{N} \cap \mathcal{D} = \emptyset$ and $\mathcal{N} \cup \mathcal{D}$ is prefix-free. $\mathcal{D}$ contains a distinguished element $*$.

$0_a$ refers to a string of ``0'' bits of length $a$, $x_{[a..b]}$ denotes a substring of $x$ consisting of bits with index $a$ through $b$ (inclusive).
$||$ denotes concatenation, $|s|$ is the length of string $s$ and $\epsilon$ is the empty string.

\subsection{Creating a mix header}
It is used as a subroutine (denoted CreateHeader) for the procedures to create forward messages and single-use reply blocks.

\emph{Input}: $(\Delta,I,\mathcal{P})$, a destination address $\Delta \in \mathcal{D}$, an identifier $I \in \{0,1\}^\kappa$ and a
sequence of mix nodes $\mathcal{P} = \{n_0,n_1,\dots,n_{\nu - 1}\}$ with $\nu \leq r$ and $|\Delta| \leq (2(r-\nu)+1)\kappa$.

Pick a random $x \in_R \mathbb{Z}_q^*$.

Compute a sequence of $\nu$ tuples $(\alpha_0,\beta_0,\gamma_0) \dots (\alpha_{\nu - 1},\beta_{\nu - 1},\gamma_{\nu - 1})$.
\begin{itemize}
  \item $\alpha_0 = g^x, s_0 = y_{n_0}^x, b_0=h_b(\alpha_0,s_0)$
  \item $\alpha_1 = g^{xb_0}, s_1 = y_{n_1}^{xb_0}, b_1=h_b(\alpha_1,s_1)$
  \item $\ldots$
  \item $\alpha_{\nu -1} = g^{xb_0b_1\dots b_{\nu -2}}, s_{\nu -1} = y_{n_{\nu -1}}^{xb_0b_1\dots b_{\nu -2}}, b_{\nu -1}=h_b(\alpha_{\nu -1},s_{\nu -1})$
\end{itemize}

The $\alpha_i$ are the group elements, the $s_i$ are the Diffie-Hellman shared secrets, and the $b_i$ are the blinding factors.


Compute the filler strings $\phi_0,\ldots,\phi_{\nu -1}$:
Let $\phi_0 = \epsilon$ and
\(\phi_i = \{\phi_{i-1}||0_{2\kappa}\} \oplus \left\{ \rho(h_\rho(s_{i-1}))_{[(2(r-i)+3)\kappa .. (2r+3)\kappa - 1]} \right\}\)
with $|\phi_i| = 2i\kappa $.

Compute a sequence of mix headers $M_{\nu - 1},M_{\nu - 2}, \dots, M_0$ with
$M_i = (\alpha_i,\beta_i,\gamma_i) \in \mathcal{G}^* \times \{0,1\}^{(2r+1)\kappa} \times \{0,1\}^\kappa$.
Let \(\beta_{\nu -1} = \{\{\Delta || I || 0_{(2(r-\nu)+2)\kappa-|\Delta|}\} \oplus \{\rho(h_\rho(s_{\nu -1}))_{[0..(2(r-\nu)+3)\kappa -1]} \}\}||\phi_{\nu-1}\).

For $0 \leq i < \nu -1$:
\begin{itemize}
  \item $\beta_i = \left\{n_{i+1}||\gamma_{i+1}||\beta_{i+1_{[0..(2r-1)\kappa -1]}} \right\} \oplus \rho(h_\rho(s_i))_{[0..(2r+1)\kappa -1]}$
  \item $\gamma_i = \mu(h_\mu(s_i),\beta_i)$
\end{itemize}

\emph{Output}: the mix header $M_0$ and the sequence of shared secrets $s_0,\dots,s_{\nu -1}$.

\subsection{Creating a forward message}
\emph{Input}: $(m,\Delta,\mathcal{P})$ a message $m$, a destination address $\Delta$ and a sequence of mix nodes $\mathcal{P} = \{n_0,n_1,\dots,n_{\nu-1}\}$ with $\nu \leq r$.

Compute mix header as above $(M_0,(s_0,\dots,s_{\nu-1})) \gets \text{CreateHeader}(*,0_\kappa,\mathcal{P})$.
Compute $\delta_{\nu-1} = \pi(h_\pi(s_{\nu-1}),0_\kappa||\Delta||m)$.
For $0 \leq i <  \nu-1$:
$\delta_i = \pi(h_\pi(s_i),\delta_{i+1})$

The forward message $(M_0,\delta_0)$ is sent to $n_0$.

\emph{Output}: the pair $(M_0,\delta_0)$.

\subsection{Creating a single use reply block}
\emph{Input}: $(\Delta,\mathcal{P})$ a destination address $\Delta$ and a sequence of mix nodes $\mathcal{P} = \{n_0,n_1,\dots,n_{\nu-1}\}$ with $\nu \leq r$.
$\Delta$ should be the user's own address.

Pick a random identifier $I \in_R \{0,1\}^\kappa$ and compute as above $(M_0,(s_0,\dots,s_{\nu-1})) \gets \text{CreateHeader}(\Delta,I,\mathcal{P})$.
Pick a random key $\tilde{k} \in \{0,1\}^\kappa$

\emph{Output}: $I$, the tuple $(\tilde{k},h_\pi(s_0),\dots,h_\pi(s_{\nu-1})))$ and the tuple $(n_0,M_0,\tilde{k})$.

\subsection{Message processing by mix nodes}
Messages received by mix nodes are of the form $(M,\delta) = ((\alpha,\beta,\gamma),\delta) \in \mathcal{G}^* \times \{0,1\}^{(2r+1)\kappa} \times \{0,1\}^\kappa \times \{0,1\}^{l_\pi}$.
The node should ensure that the message is in this form; in particular, that $\alpha \in \mathcal{G}^*$.
When mix node $n$, with private key $x_n$, receives such a message, it proceeds as follows:

Compute a shared secret $s = \alpha^{x_n}$.
If $h_\tau(s)$ is already in this node's table of seen message tags, discard the message.
Otherwise, continue by comparing $\gamma$ to $\mu(h_\mu(s),\beta)$
If they do not match, discard the message.
Otherwise, store $h_\tau(s)$ in the table of seen message tags.
Decrypt padded $\beta$ to get $B = \{\beta||0_{2\kappa}\} \oplus \rho(h_\rho(s))$.

Parse prefix of $B$ as $n \in \mathcal{N} \cup \mathcal{D}$.
If this is not possible, discard the message.

\begin{itemize}
  \item $n \ in \mathcal{N}$: The message is destined for another Sphinx node. Compute the blinding factor $b=h_b(\alpha,s)$. Let $\alpha' = \alpha^b$, $\gamma' = B_{[\kappa..2\kappa-1]}$, $\beta' = B_{[2\kappa..(2r+3)\kappa-1]}$ and $\delta'=\pi^{-1}(h_\pi(s),\delta)$. Send $((\alpha',\beta',\gamma'),\delta')$ to $n$.
  \item $n = *$: The current node is the exit node for a forward message. Let $\delta' = \pi^{-1}(h_\pi(s),\delta)$. If $\delta'_{[0..\kappa-1]} = 0_\kappa$, parse $\delta'_{[\kappa..l_\pi-1]}$ as $\Delta||m$ for $\Delta \ in \mathcal{D}$. If successful, $\Delta$ should be a plaintext message and is sent to $\Delta$. Otherwise, the message has been tampered with and is discarded.
  \item $n \in \mathcal{D} \setminus\{*\}$: The current node is the exit node for a reply message. $n$ is the owner of a pseudonym. Let $I = B_{[|n|..|n|+\kappa-1]}$ and $\delta' = \pi^{-1}(h_\pi(s),\delta)$. Send $(I,\delta')$ to $n$.
\end{itemize}


==> sections/OSDefinitions.tex <==
\subsubsection{Honest Sender to Honest Node}\label{sec:honestSenderToHonestNodeDef}
\begin{definition}{$\OSSenderNode$}\footnotesize \label{def:OSSenderNode}
\begin{enumerate}
\item The adversary receives as input the challenge public keys $PK$, chosen by the challenger by letting $(PK, SK) \gets G(1^\lambda , p)$, and the router name $P$.
\item The adversary may submit any number of onions $O_i$ of her choice to the challenger.
The challenger sends the output of $\mathrm{ProcOnion}(SK, O_i , P )$ to the adversary.
\item The adversary submits an original message $m$, an original path $\mathcal{P}=(P_1 , \dots, P_j, \dots, P_{n+1})$ with the honest node at position $j$,$1 \leq j \leq n + 1$ of her choice, a modification function $f$ for the onion before entering the honest relay
and key pairs for all nodes $(PK_i , SK_i )$ ($1\leq i \leq n+1$ for the nodes on the path and $n+1<i$ for the other relays). The challenger checks that the router names are valid, that the public keys correspond to the secret keys and that the same key pair is chosen if the router names are equal, and if so, sets $PK_{j} = PK$, sets bit $b$ at random, and does create the onion as the adversary's input choice:
  \begin{align*}
    ({O}_1,  \dots, {O}_{n+1})\gets \mathrm{FormOnion}(&m, \mathcal{P}, (PK)_{\mathcal{P}})
  \end{align*}
  \item The challenger creates a random onion with a randomly chosen fake path $\bar{\mathcal{P}}=(\bar{P}_1=P_1 , \dots,\bar{P}_j=P_j, \bar{P_{j+1}} ,\dots, \bar{P}_{\bar{n}+1})$, that includes the subpath from the honest sender to  honest node of $\mathcal{P}$  starting at position $1$ ending at $\bar{j}=j$  (honest node $\bar{j}$ with $1 \leq \bar{j} \leq \bar{n} + 1$) and matches the path properties, and a random message $m'$:
     \begin{align*}
    ({\bar{O}}_1,  \dots, {\bar{O}}_{\bar{n}+1})\gets \mathrm{FormOnion}(&{m'},\bar{\mathcal{P}}, (PK)_{\bar{\mathcal{P}}})
  \end{align*}
\item 
	\begin{itemize}
		\item If $b = 0$, the challenger gives $(O_1,ProcOnion(f(O_{j})))$ to the adversary.
		\item Otherwise, the challenger gives $(\bar{O}_1, ProcOnion(f(O_{j})))$ to the adversary.
	\end{itemize}
\item Now the adversary is allowed to get responses for this type of queries: Submit any onion $O_i$, $O_i \noduplicate f(O_j)$, $O_i \noduplicate f(\bar{O}_j)$
 of her choice. 
\item The adversary then produces a guess $b'$ .
\end{enumerate}
\end{definition}

\subsubsection{Between Honest Nodes}\label{sec:betweenHonestNodesDef}

\begin{definition}{$\OSNodeNode$}\footnotesize \label{def:OSNodeNode}
\begin{enumerate}
\item The adversary receives public keys $PK_1, PK_2$, chosen by the challenger by letting $(PK_j, SK_j) \gets G(1^\lambda , p)$ for $j \in \{1,2\}$, and router names $P_1,P_2$.
\item The adversary may submit any number of onions $O_i$ and router names $P_j$; $j \in \{1,2\}$, of her choice to the challenger.
 and gets the output  of $\mathrm{ProcOnion}(SK_j, O_i , P_j)$ to the adversary.
\item The adversary submits an original message $m$, an original path $\mathcal{P}=(P_1 , \dots, P_{j_1} \dots, P_{j_2} , P_{n+1})$ with the honest nodes at positions $j_1, j_2$, with $1 \leq j_1<j_2 \leq n + 1$, and a modification function $f_j'$ for the onion before entering the  $j'$-th honest relay
and key pairs for all nodes $(PK_i , SK_i )$ ($1\leq i \leq n+1$ for the nodes on the path and $n+1<i$ for the other relays). The challenger checks that the router names are valid,  that the public keys correspond to the secret keys and that the same key pair is chosen if the router names are equal, and if so, sets $PK_{j} = PK$, sets bit $b$ at random, and does the following:
  \begin{align*}
    ({O}_1,  \dots, {O}_{n+1})\gets \mathrm{FormOnion}(&m, \mathcal{P}, (PK)_{\mathcal{P}}) 
     \end{align*}
  \item The challenger creates a random onion with a fake path $\bar{\mathcal{P}}=(\bar{P}_1 ,\dots, \bar{P}_{\bar{j_1}}=P_{j_1},\dots,\bar{P}_{\bar{j_2}}=P_{j_2}, \dots, \bar{P}_{\bar{n}+1})$, matching the modified onion in the faked part of communication, i.e. that includes the subpath from the first honest  to the second honest node of $\mathcal{P}(f_1(O_{j_1}))$\footnote{If $\mathcal{P}(f_1(O_{j_1}))$ does not include the second honest node, the challenger aborts.}  starting at position $\bar{j_1}$ ending at $\bar{j_2}$  (honest nodes $\bar{j_1}, \bar{j_2}$ with $1 \leq \bar{j_1}<\bar{j_2} \leq \bar{n} + 1$) and matches the path properties, and a random message $m'$:
     \begin{align*}
      ({\bar{O}}_1,  \dots, {\bar{O}}_{\bar{n}+1})\gets \mathrm{FormOnion}(&{m'},\bar{\mathcal{P}}, (PK)_{\bar{\mathcal{P}}})
  \end{align*}
\item Depending on $b$ the challenger returns:  
	\begin{itemize}
		\item If $b = 0$, the challenger returns $(O_1,$ $ProcOnion(f_1(O_{j_1})),$ $ProcOnion(f_2(ProcOnion^{j_2}(f_1(O_{j_1}))) )$\footnote{$ProcOnion^{j_2}$ means processed until before node $P_{j_2}$}
		\item Otherwise, the challenger returns $( O_1,$ $\bar{O}_{{\bar{j}_1}+1},$ $ProcOnion(f_2(ProcOnion^{j_2}(f_1(O_{j_1}))) )$
	\end{itemize}
\item Now the adversary is allowed get responses for this type of queries: Submit any onion $O_i$  and router names $P_k$; $k \in \{1,2\}$ and , $O_i \noduplicate f(O_{j_k})$, $O_i \noduplicate f(\bar{O}_{j_k})$ of her choice. The challenger 
sends the output of $\mathrm{ProcOnion}(SK_j, O_i , P_j)$ to the adversary. 
\item The adversary then produces a guess $b'$ .
\end{enumerate}
\end{definition}


\subsubsection{Honest Node to Receiver}\label{sec:honestNodeToReceiverDef}

\begin{definition}{$\OSNodeReceiver$}\footnotesize \label{def:OSNodeRec}
\begin{enumerate}
\item The adversary receives as input the challenge public keys $PK$, chosen by the challenger by letting $(PK, SK) \gets G(1^\lambda , p)$, and the router name $P$.
\item The adversary may submit any number of onions $O_i$ of her choice to the challenger. The challenger sends the output of $\mathrm{ProcOnion}(SK, O_i , P )$ to the adversary.
\item The adversary submits message $m$, an original path $\mathcal{P}=(P_1 , . . . , P_{n+1})$ with the honest node at position $j$,$1 \leq j \leq n + 1$, and a modification function $f$ for the onion before entering the honest relay
and key pairs for all nodes $(PK_i , SK_i )$ ($1\leq i \leq n+1$ for the nodes on the path and $n+1<i$ for the other relays).
 The challenger checks that the router names are valid,  that the public
keys correspond to the secret keys and that the same key pair is chosen if the router names are equal, and if so, sets $PK_{j} =  PK$, sets bit $b$ at random, and does the following:
  \begin{align*}
    ({O}_1,  \dots, {O}_{n+1})\gets \mathrm{FormOnion}(&m, \mathcal{P}, (PK)_{\mathcal{P}})
  \end{align*}
    \item The challenger creates a random onion with a randomly chosen fake path $\bar{\mathcal{P}}=(\bar{P}_1=P_1 , \dots,\bar{P}_j=P_j, \bar{P_{j+1}} ,\dots, \bar{P}_{\bar{n}+1})$, that includes the subpath from the honest relay to  the receiver of  $\mathcal{P}(f(O_j))$  starting at position $j$ ending at $n+1$ (honest node $\bar{j}$ with $1 \leq \bar{j} \leq \bar{n} + 1$) and matches the path properties:
     \begin{align*}
    ({\bar{O}}_1,  \dots, {\bar{O}}_{\bar{n}+1})\gets \mathrm{FormOnion}(&{m},\bar{\mathcal{P}}, (PK)_{\bar{\mathcal{P}}})
  \end{align*}
  \item
	\begin{itemize}
		\item If $b = 0$, the challenger gives $(O_1, ProcOnion(f(O_{j})))$ to the adversary
		\item Otherwise, the challenger gives $({O}_1, ProcOnion(\bar{O}_{j}))$ to the adversary
	\end{itemize}
\item Now the adversary is allowed get responses for this type of queries: Submit any onion $O_i$, $O_i \noduplicate f(O_j)$, $O_i \noduplicate \bar{O}_j$ of her choice. 
The challenger sends the output of $\mathrm{ProcOnion}(SK_j, O_i , P_j)$ to the adversary. 
\item The adversary then produces a guess $b'$ .
\end{enumerate}
\end{definition}

==> sections/camenischBackgroundProperties.tex <==
\subsubsection{Properties}\label{secBG:properties}
\cite{camenisch2005formal} defines three properties and claims that they imply the ideal functionality. Later works split one of the properties in two. 
The resulting four properties are onion-correctness, onion-integrity, onion-security and  wrap-resistance.

Informally, \emph{onion-correctness} requests that all messages use the intended path and reach the intended receiver in absence of an adversary:\todo{I slightly changed the definition to get rid of other definition it referenced. how to show this?i.a.w.?}
\begin{definition}[Onion-correctness i.a.w.~\cite{camenisch2005formal}] \label{def:onionCorrectnessOrig}
Let \((G, \FormOnion, \ProcOnion)\) be an \ac{OR} scheme with maximal path length $N$.
Then  for all polynomial number of routers $P_i$, for all settings of the public parameters $p$, for all $(PK(P),SK(P))$ generated by $G(1^\lambda, p, P)$, 
for all $n < N$,
%for any path $P = (P_1 , . . . , P_{n+1} )$,
% and for all sets with a polynomial number of honest router names $Q$ with a public-key infrastructure ($(PK(P),SK(P))$ generated by $G(1^\Lambda, p, P)$ for $P \in Q$), for any path $P = (P_1 , \ldots , P_{n+1} )$, \todo{no  $P \subseteq Q$}%$P \subseteq Q$, 
for all messages
$m \in \mathcal{M}$, and for all onions $O_1$ formed as 
{\center
  $ \displaystyle
    \begin{aligned} 
(O_1, \dots , O_{n+1} )\gets &\FormOnion(m, (P_1 , \dots , P_{n+1} ), \\
&(PK(P_1 ), \ldots , PK(P_{n+1} )))
    \end{aligned}
  $ 
\par}
the following is true: 
\begin{enumerate}\small
\item  correct path: \(\mathcal{P}(O_1, P_1) = (P_1, \ldots , P_{n+1} )\),
\item correct layering: \(\mathcal{L}(O_1 , P_1 ) = (O_1 , \ldots , O_{n+1})\),
\item correct decryption:\\  \((m, \perp) = \ProcOnion(SK(P_{n+1} ), O_{n+1}, P_{n+1}) \),
\end{enumerate}\small
where $\mathcal{P}(O,P)$ returns the path included in $O$ and $\mathcal{L}(O,P)$ the onion layers.
\end{definition}
\vspace{0.15cm}

\emph{Onion-Integrity} limits the number of honest relays that any onion (even one created by the adversary) can traverse.
\begin{definition}[Onion-integrity i.a.w.~\cite{camenisch2005formal}]\label{def:onionIntegrity}
For all \ac{PPT} adversaries, the probability (taken over the choice of the public parameters \(p\), the set of honest router names \(\mathcal{Q}\) and the corresponding PKI, generated by $G$) that an adversary with adaptive access to \(\mathrm{ProcOnion}(SK(P ), \cdot, P )\) procedures for all \(P \in \mathcal{Q}\), can produce and send to a router \(P_1 \in \mathcal{Q}\) an onion \(O_1\) such that \(|\mathcal{P}(O_1,P_1)| > N\), is negligible.
\end{definition}
\vspace{0.15cm}

\emph{Onion-security} states that an adversary cannot distinguish an onion created with self-chosen inputs (except for the keys of one honest node) from another onion whose message and path after an honest node differ. Therefore the adversary is even allowed to observe the processing of any other onion at the honest node via an oracle.
\begin{definition}[Onion-Security i.a.w.~\cite{camenisch2005formal}]\label{def:onionSecurity}
  Consider an adversary interacting with an \ac{OR} challenger as follows.
  \begin{enumerate} \small
   \item The adversary receives as input a challenge public key \(PK\), chosen by the challenger by letting \((PK,SK) \leftarrow G(1^{\lambda}, p)\), and the router name \(P\).
    \item The adversary submits any number of onions \(O_i\) of her choice to the challenger, and obtains the output of \(\mathrm{ProcOnion}(SK, O_i, P)\).
    \item The adversary submits \(n\), a message \(m\), a set of router names \((P_1,\ldots,P_{n+1})\), an index \(j\), and \(n\) key pairs \(1 \leq i \leq n, i \neq j, (PK_i, SK_i)\).
      The challenger checks that the router names are valid, that the public keys correspond to the secret keys and if so, sets \(PK_j = PK\), sets bit \(b\) at random and does the following:
      \begin{itemize}
        \item If \(b=0\), let
          \((O_1,\ldots,O_j,\ldots,O_{n+1}) \leftarrow \mathrm{FormOnion}(m,(P_1,\ldots,P_{n+1}),(PK_1,\ldots,PK_{n+1}))\)
        \item Otherwise, choose \(r \leftarrow \mathcal{M}\), and let
          \((O_1,\ldots,O_j) \leftarrow \mathrm{FormOnion}(r,(P_1,\ldots,P_{j}),(PK_1,\ldots,PK_{j}))\)
      \end{itemize}
      The challenger returns \(O_1\) to the adversary.
          \item The adversary may submit any number of onions \(O_i \neq O_j\) of her choice to the challenger, and obtain the output of \(\mathrm{ProcOnion}(SK, O_i, P)\).
    \item The adversary then produces a guess $b'$.
  \end{enumerate}
        
  An \ac{OR} scheme satisfies onion security if for all \ac{PPT} adversaries \(A\), there is a negligible function \(v\) such that the adversary's probability of outputting $b'=b$ is at most \(\frac{1}{2}+v(\lambda)\).
\end{definition}
\vspace{0.15cm}


\emph{Wrap-resistance} informally means that given an onion, which resulted from processing at a certain relay, the adversary cannot add a layer to it, such that processing at another relay results in the same onion. 

\begin{definition}[wrap-resistance i.a.w.~\cite{camenisch2005formal}]\label{def:wrapResistance}
  Consider an adversary interacting with an \ac{OR} challenger as follows.
 
  \begin{enumerate}\small
       \item - 4) as in Definition~\ref{def:onionSecurity}
    \addtocounter{enumi}{3}
    \item The adversary submits a secret key \(SK'\), an identity \(P' \neq P_{j-1}\), and an onion \(O'\).
      If \(P'\) is valid and \(SK',O',P'\) satisfy the condition \(O_j=\mathrm{ProcOnion}(SK',O',P')\) he wins the game.
  \end{enumerate}
    
  An \ac{OR} scheme satisfies wrap-resistance if for all \ac{PPT} adversaries \(A\) the adversary's probability of winning is negligible.
\end{definition}


==> sections/correctedProofStep.tex <==
\begin{claim}
Consider a family of hybrids: $\mathcal{H}^k$ runs like $\mathcal{H}_0$ until the $k$-th time the conditions (1) and (2) from $\mathcal{H}_1$ are met. At this point it starts behaving like $\mathcal{H}_1$.  For any $k$, that is a poly function of $\lambda$: $\mathcal{H}^k$ and $\mathcal{H}^{k-1}$ are indistinguishable.
\end{claim}

\begin{proof}
%\todo[inline]{From my notes: we know whether the $k$-th meeting of the condition is the original or the randomly chosen message, which equals the challenge bit in onion security.}
(indirect) We assume, the adversary can distinguish $\mathcal{H}^k$ and $\mathcal{H}^{k+1}$. That implies that it exists an attacker $A_H$ that communicates with the machine $\mathcal{H}$ in question, such that it exists an successful distinguisher $D$, that acts as the environment for $\mathcal{H}$. $D$ being successful means: \[Pr(D \text{ guesses correct})\geq \frac{1}{2} + \epsilon \text{ for some non-negligible }  \epsilon \text{,}\] 
where the correct guess for $\mathcal{H}^{k+1}$ is 1 and for $\mathcal{H}^{k}$ is 0.

The adversary $A_{os}$uses $D$ to break onion security by constructing a machine $\mathcal{H}^A$ whose output to $D$ is indistinguishable from $\mathcal{H}^k$'s if  onion-security challenge bit $b=0$ and from $\mathcal{H}^{k+1}$ if $b=1$ with non-negligible probability:

\textbf{Attack description}
Step 1 of onion security (OS) game: The adversary receives a public key $PK$ and router name $P$ from the onion security challenger $Ch_{os}$.  
$\mathcal{H}^A$ runs the setup like $\mathcal{H}_0$  and stores all key-pairs $(PK_i,SK_i)$. Then it sets the $PK$ for $P$. It does not need to generate the belonging secret key $SK$ for $P$. Instead, whenever $SK$ is needed, it communicates with the adversary $A_{os}$, who in turn uses the procOnion oracle from $Ch_{os}$ (Step 2 or 4 of OS game). 
$\mathcal{H}^A$ communicates with $D$ and $A_H$ like $\mathcal{H}_0$, but additionally counts how often the condition of $\mathcal{H}_1$ are met until they are met for the $k-1$-th time. 

When the conditions would be met for the $k$-th time, $\mathcal{H}^A$ creates a copy of its own state and continues the run $\mathcal{H}_0$ until the onion responsible for the $k$-th matching of conditions is handed to its receiver without giving output to $D$ or $A$.\footnote{Since we control $\mathcal{H}^A$, we can do this} This way, $\mathcal{H}^A$ learns the path $P_1,\dots ,P_n$ and the message $m$ of the onion $O_H$. By definition of $\mathcal{H}_1$ $P_2=P_{o_{i+1}}$ is an adversarial node, let $P_j$ be the smallest $j>2$, such that $P_j$ is honest (such $P_j$ has to exist by definition of $\mathcal{H}_1$). If $P_j \neq P$, $A_{os}$ outputs a random guess $b'$. 

Otherwise($P_j = P$),%$\mathcal{H}_A$ uses procOnion to unpeal $O_H$ to the onion $m$ it is, when  it reaches $P_j$ by using procOnion and the secret keys. 
$A_{os}$ hands $(P_2,\dots, P_n),j-1, m$ and $(SK_i,PK_i)$ to $Ch_{os}$ and receives onion $O$ as answer. Now the other copy of $\mathcal{H}^A$ runs with outputs for $D$, onion $O_H$ one step to $P_2$. Then the challenge onion $O$ is input to $P_2$ and run for the path until before it arrives at $P_j$. $\mathcal{H}^A$ sees when it would be sent to $P_j$ and replaces it at this point with $O_H'$, which is $O_H$ pealed until right before procOnion of $P_j$.

Further on $\mathcal{H}^A$ runs like $\mathcal{H}_1$ and communicates with $D$. Once $D$ decides on an output, $A_{os}$ guesses the negated  bit $b'=D(\mathcal{H}^A)$.

\textbf{Attack analysis}
If onion security challenge bit $b=0$ and $P$ is $P_j$: The challenger returns onion $O$, that includes the real message $m$ for $P_n$. Since we insert this onion for $P_2$, it will go its way just like $O_H$ would until before $P_j$. There it is replaces with $O_H'$, that continues the last part of the path just as $O_H$ would have. Hence, the behavior and the output of machine $\mathcal{H}^A$ for the $k$-th time the conditions are met is the same as $\mathcal{H}_0$. Before it behaves like $\mathcal{H}_0$ and afterwards like $\mathcal{H}_1$. Hence it behaves like $\mathcal{H}^{k+1}$.

If onion security challenge bit $b=1$ and $P$ is $P_j$: The challenger returns onion $O$, that includes a random message $r$ for $P_j$ and this onion is input to $P_2$ by $\mathcal{H}_A$. Before it arrives at $P_j$, $\mathcal{H}_A$ replaces it with $O_H'$ that goes through the remaining nodes of the path just as $O_H$ would have. Hence, in the $k$-th time the conditions are met $\mathcal{H}_A$ behaves like $\mathcal{H}_1$. Before it behaves like $\mathcal{H}_0$ and afterwards like $\mathcal{H}_1$. Hence it behaves like $\mathcal{H}^{k}$.

Advantage of $\mathcal{H}^{A}$:
Let $n$ be the number of  onion routers $P_1, \dots, P_n$.
\begin{align*}
Pr(b'=b) &= Pr(P=P_j) \cdot Pr(b'=b\mid P= P_j) +  Pr(P  \neq P_j) \cdot Pr(b'=b\mid P\neq P_j)\\
&= \frac{1}{n} \cdot Pr(b'=b\mid P= P_j) +  \frac{n-1}{n} \cdot \frac{1}{2}\\
&= \frac{1}{n} \cdot Pr(D \text{ guesses correct}) +  \frac{n-1}{n} \cdot \frac{1}{2}\\
&\geq \frac{1}{n} \cdot (\frac{1}{2}+ \epsilon) +  \frac{n-1}{n} \cdot \frac{1}{2}\\
&= \frac{1}{2} + (\frac{1}{n} \cdot \epsilon)\\
\end{align*}

$\frac{1}{n} \cdot \epsilon$ is non-negligible, since per assumption $\epsilon$ and $\frac{1}{n}$ are non-negligible. 

\end{proof}


This claim implies ``The view with $\mathcal{H}_0$ is indistinguishable from the view with $\mathcal{H}_1$'' as needed for the proof of Theorem 1 in  \cite{camenisch2005formal}.

\paragraph{Unexpected Results}
With this, the proof is never using the wrap resistance part of onion security. Hence, to achieve the ideal functionality, it is not needed.


==> sections/framework.tex <==
We use the framework of Kuhn et al.~\cite{ownFramework} that unifies the privacy goals of existing theoretical analysis frameworks~\cite{backes2017anoa, bohli_relations_2011, gelernter_limits_2013, hevia_indistinguishability-based_2008}, like the established AnoA-Framework~\cite{backes2017anoa}. \cite{ownFramework}  introduces a well-analyzed hierarchy of privacy goals and thus allows our analysis results for \ac{OR} to be easily comparable.

\subsubsection{Privacy Goals}
The basic idea  of the analysis is to challenge the adversary to distinguish two simulations of the protocol that differ only in protected parts of the communications (e.g. who the sender of a certain message was). The communications input for the two simulations are called scenarios and are chosen by the adversary to reflect the worst case. A communication contains a sender, receiver, message and auxiliary information, like for our purpose the path included in the onion. The \emph{privacy notion} specifies how the communications of the scenarios are allowed to differ.

Formally, the model uses $r=(u,u',m,aux)$ to denote the communication of message $m$ from sender $u$ to receiver $u'$ with auxiliary information $aux$. Communications that are processed together are grouped in batches $\underline{r}$. For the game the adversary has to decide on two scenarios. Those are a sequence of pairs of batches. The challenger verifies for every pair of  batches $\underline{r}_0, \underline{r}_1$  that they comply to the currently analyzed privacy notion, i.e. differ only in private information. If the pair of batches is valid regarding the notion, the challenger picks a random $b$ and simulates the protocol for the corresponding batch $\underline{r}_b$. Then the adversary can issue more valid batches and finally has to make a guess $g$ for $b$. If any adversary cannot achieve a better probability of guessing $g=b$ correctly as negligibly bigger than $\frac{1}{2}$, the notion is achieved as nothing about the private information can be learned. 

We are especially interested in four privacy notions. 
The first is a strong form of confidentiality. It states that the adversary is not able to decide which of two self-chosen messages was sent in the simulation. As thus the message is unobservable, it is called \emph{Message Unobservability} ($\conf$). 
The second was already introduced in our example with Alice and Bob and is a form of sender anonymity. There, informally speaking, the adversary is not able to decide  for even one of  her self-chosen senders which of her self-chosen messages it sent. As thus she cannot link the sender to its message, this notion is called \emph{Sender-Message Unlinkability} ($\SML$). 
The third, analogous to the second, is a form of receiver anonymity. This time, the adversary is not able to decide  for even one of  her self-chosen receivers which of her self-chosen messages it received. As thus she cannot link the receiver to its message, this notion is called \emph{Receiver-Message Unlinkability} ($\RML$). 
The fourth is a form of relationship anonymity. There the adversary is not able to decide which pairings of two self-chosen senders and two self-chosen receivers communicated with each other. 
As thus she cannot link the sender to the receiver, this notion is called \emph{Sender-Receiver Unlinkability} ($\PairSRL$\footnote{This notion is named $(SR)\overline{L}$ in~\cite{ownFramework}.}).
 
 To keep the formal definitions of the notions short, we always consider the following:
 Let the checked batches be $\underline{r_0},\underline{r_1}$,  which  for $b \in \{0,1\}$ include the communications \mbox{${r_b}_j = (u_{b_j},u'_{b_j},m_{b_j},aux_{b_j})$} with $ j \in \{1, \dots l\} $. 

 For $\conf$ two batches may only  differ in the messages:
\begin{definition}[$\conf$ i.a. w. \cite{ownFramework}]
The batches are valid for $\conf$, iff for all $j \in \{1, \dots l\}$:  ${r_1}_j =(u_{0_j},u'_{0_j},\mathbf{m_{1_j}},aux_{0_j}) $. 
\end{definition}

For $\SML$ only the senders may differ and further each sender has to send the same number of messages in the two batches. To define this, \cite{ownFramework} formally defines $Q_b$. Here we use a less formal description: \(Q_b:=\{(u,n)\mid u \text{ sends } n \text{ messages in } \underline{r}_b\}\).
\begin{definition}[$\SML$ i.a. w. \cite{ownFramework}]
The batches are valid for $\SML$, iff for all $j \in \{1, \dots l\}:{r_1}_j =(\mathbf{u_{1_j}},u'_{0_j},m_{0_j},aux_{0_j})$ and $Q_0=Q_1$.
\end{definition}

$\RML$ is analogous to $\SML$, but for receivers:  \(Q_b':=\{(u',n)\mid u' \text{ receives } n \text{ messages in } \underline{r}_b\}\).
\begin{definition}[$\RML$ i.a. w. \cite{ownFramework}]
The batches are valid for $\RML$, iff for all $j \in \{1, \dots l\}:{r_1}_j =(u_{0_j},\mathbf{u'_{1_j}},m_{0_j},aux_{0_j})$ and $Q_0'=Q_1'$.
\end{definition}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.17\textwidth]{Images/MSR.pdf}
  \caption{Batches in $M_{SR}$ illustrated}
  \label{fig:MSR}
\end{figure}

$\PairSRL$ allows only sender and receiver to differ and has the complex requirement $M_{SR}$. $M_{SR}$ is defined formally in~\cite{ownFramework} and requires that two senders and receivers in both batches are mixed in the following way: The batches only differ in two senders ($A,C$) and two receivers ($B, D$). In the case $b=0$: $A$ must communicate with $B$, and $C$ with $D$; in the case $b=1$: $A$ with $D$, and $C$ with $B$. The order of those two communications in the batch is chosen randomly by the challenger. Before, between and after those communications multiple communications that are equal in both batches can occur. The possible communications are depicted in Fig. \ref{fig:MSR}.
\begin{definition}[$\PairSRL$ i.a. w. \cite{ownFramework}]
The batches are valid for $\PairSRL$, iff for all $j \in \{1, \dots l\}:{r_1}_j =(\mathbf{u_{1_j}},\mathbf{u'_{1_j}},m_{0_j},aux_{0_j})$ and $M_{SR}$.
\end{definition}

\subsubsection{Corruption}
Further, we want to look at different kinds of user (sender and receiver) corruption. All the notions exist can be analyzed under different allowed corruption. Therefore, options for user corruption are defined and added to the abbreviation of any privacy notion $X$.
We look at the following cases:  
\begin{itemize}
\item [$\noCorr{X}$:] no users are corrupted, but some relays or links can be,
\item  [$\corrOnlyPartnerSender{X}$:] only receivers, but no senders are corrupted, and
\item [$\corrStandard{X}$:] corrupted users can be senders and receivers, but they send/receive the same messages in both simulations.
\end{itemize}
 Note that $\corrStandard{X}$ is needed as otherwise the notion can be broken by observing the behavior of corrupted users.
 
 Formally, corruption is realized with special corrupt-queries. They return internal information of the corrupted user (keys, current state etc.). $X_{c^0}$ ensures that the adversary is not allowed to send any corrupt-query. The other corruption options add requirements for the two batches of the adversary to be considered valid.
\begin{definition}[Corruption]\label{def:corruption}
Let $\hat{U}$ be the set of all users corrupted via corrupt-queries.
The following corruption options are met, iff for all $a \in \{0,1\}$:
{\footnotesize
\begin{align*}
  \corrOnlyPartnerSender{X}&: \forall (u,u',m,aux) \in \underline{r}_0\cup \underline{r}_1: u \not \in \hat{U} \\
  \corrStandard{X}&: \forall \hat{u} \in \hat{U}:r_{0_i}=(\hat{u},\_,m,\_) \implies r_{1_i}=(\hat{u},\_,m,\_)\\
   &\quad \quad \quad \quad \land r_{0_i}=(\_,\hat{u},m,\_) \implies r_{1_i}=(\_,\hat{u},m,\_) \\
\end{align*}
}
\end{definition}

The specific adversary model, e.g. how many relays can be corrupted, used for the analysis is adjustable by the adversary class. An adversary class can filter and modify the adversary chosen scenarios before they are input into the protocol simulation or ideal functionality.

\subsubsection{Relation of Goals}
As a side benefit, our analysis allows statements even for notions we did not directly analyze: By showing that a certain notion is achieved by the analyzed protocol all the weaker notions are shown to be achieved as well. We say that the weaker notions are implied by the stronger one. The same holds true for dependencies between corruption. 
As we not only want to prove that the introduced notions are achieved, but also that they are the strongest achievable by using only \ac{OR}, we show attacks for the stronger notions. The according part of the hierarchy is illustrated in Fig. \ref{fig:hierarchy} and the analyzed notions are highlighted. The notions  for which we show that they are not achieved  are introduced in Appendix \ref{app:notionDef} due to space limitations.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.48\textwidth]{Images/hierarchy.pdf}
  \caption{Excerpt of the hierarchy of~\cite{ownFramework}}
  \label{fig:hierarchy}
\end{figure}


==> sections/globalActive.tex <==
We analyze the original ideal functionality $\originalIdeal$ according to the privacy goals. Therefore we use \cite{ourFramework} and allow the path $\mathcal{P}$ to be specified in the auxiliary information. Since in \cite{ourFramework} the game adversary picks the communications of both scenarios, it could always choose paths only consisting of adversarial relays. However, for an honest sender we want to be able to model a different choice of the path. Hence, we use an adversary class, that checks the specified user corruption (e.g. honest sender, but corrupted receiver) and additionally replaces the adversary chosen paths with other paths, whenever a honest sender constructs the onion. Those other paths are randomly chosen. \todo{such that they include at least one honest node?} We call those adversary classes $C_{P,c^{\text{corruption option}}}$ (C for Class, P for Path change and c for corruption of users.).

\begin{theorem}
$\originalIdeal$ achieves $\conf$ for adversary class $C_{P,c^{R}}$. \label{TheoremConf}
\end{theorem}

\begin{proof}
We go through the messages of the ideal functionality $\originalIdeal$ and check whether they help to distinguish two scenarios differing only in the messages.

\emph{Process\_New\_Onion:} Does not output anything to the adversary and is used only by the challenger to model the start of the communication.
  
\emph{Process\_Next\_Step:} Since the receiver are not allowed to be corrupted ( $C_{P,c^{R}}$), the adversary only gets messages ``Onion temp from $P_{o_i}$ routed through ($P_{o_{i+1}}, \dots, P_{o_{j-1}}$ to $ P_{o_j}$)'' or  ``Onion temp from $P_{o_i}$ to $P_{o_{i+1}}$''. Since everything except the messages is equal in both scenarios, the path is equal in both scenarios and does not help the adversary distinguish. Further $temp$ is generated randomly  by $\originalIdeal$  and hence does not help the adversary distinguish.

\emph{Deliver\_Message:} The adversary can decide to relay some onions. However, since the onions are taking the same path in both scenarios and their $temp$ is random the adversary cannot deduce anything about the message, even if she delays some onions.

\emph{Forward\_Onion:}  Is a message between honest routers and the ideal functionality. Hence, the adversary cannot influence it or get information from it.
\end{proof}

\todo[inline]{This is somewhat strange, since the ideal functionality does not leak the message's length, but the later used ideal functionality for secure point-to-point channels does! This implies quite some privacy goals of our hierarchy, which makes it not so easy to sell...}

\begin{theorem}
$\originalIdeal$ does not achieve any notion (of the hierarchy in \cite{ourFramework}) not implied by $\conf$ for adversary class  $C_{P,c^{R}}$.
\end{theorem}

\begin{proof}
We need to show, that $\mathcal{F}$ does not achieve any of the lowest notions in the hierarchy that are not already implied by $\conf$ for  $C_{P,c^{R}}$:  $\PairSRL$, $\SRO$, $\PairSL$, $\PairRL_{c^0}$ for  $C_{P,c^{0}}$. With this shown, it follows that also no stronger notion than $\conf_{c^{R}}$ can be achieved, even without corruption.
Further, we show, that with receiver corruption allowed it also does not achieve $\PairSML$,$\SMO$,$\PairRML$,$\RMO$ for  $C_{P,c^{S}}$.
With this shown, it is clear that with corrupted receivers also no $\conf$ for  $C_{P,c^{S}}$ can be achieved.

\item  $\PairSRL$ for  $C_{P,c^{0}}$:
 
 The attack works as follows: We use the two communications from two pairs of users $A\rightarrow B$, $C \rightarrow D$ as the first instance of the first scenario and the others according to the definition of $\PairSRL$ (see Figure \ref{fig:senderReceiver} a).
 
 Now, the ideal functionality $\mathcal{F}$ will output ``Onion temp from $A$ to $X$'' and ``Onion $temp'$ from $C$ to $X'$ ''. We will use $Deliver\_Message$ for $temp$ and continue getting messages ``Onion $\overline{temp}$ from $X_1$ to $X_2$'' and using $Deliver\_Message$ for $\overline{temp}$ until we get a message ``Onion temp from $X_1$ to $B$'' or ``Onion temp from $X_1$ to $D$''. If it is $B$, we guess that $g=0$, otherwise we guess $g=1$.
 \todo[inline]{who picks the path? attacker? random?}
\begin{figure}[htb]
  \centering
  \includegraphics[width=0.48\textwidth]{Images/complexProp.pdf}
  \caption{Examples showing the general structure of communications that differ in both scenarios: a) Naive, but incorrect b) Random Sender Receiver $R_{SR}$ c) Mixed Sender Receiver $M_{SR}$}
  \label{fig:senderReceiver}
\end{figure}

\item $\SRO$ for  $C_{P,c^{0}}$:

Same attack as $\PairSRL$ for  $C_{P,c^{0}}$, except that we only observe either $A$ or $C$ as sender, either $B$ or $D$ as receiver and need to input the communications from Figure \ref{fig:senderReceiver} b as our attack to be valid for $\SRO$.

\item  $\PairSL$ for  $C_{P,c^{0}}$ ($\PairRL$ analogous):

Use senders $A$ and $C$ for the two instances of the two scenarios according to Figure \ref{fig:senderReceiver} c. In this case, we do not need to use $Deliver\_Message$ even once; we just wait for the first messages the ideal functionality sends in $Process_Next_Step$ ``Onion temp from $S_1$ to $X$'' and ``Onion temp from $S_2$ to $X$'', if those two senders are the same, we guess $g=0$, otherwise $g=1$.

\item $\PairSML$ for  $C_{P,c^{S}}$:

As above in the case for  $\PairSRL$ for  $C_{P,c^{0}}$ we get the senders linked to the first $temp$ by the first message of the ideal functionality to us (the adversary). We decide on one of the senders and only use $Deliver\_Message$ for its $temp$ and all the $\bar{temp}$ that we get later (except of course the $temp'$ that we linked to the other sender. As we are allowed to corrupt the receiver, we (of course) pick a corrupted receiver $r$. Hence, we continue using $Deliver\_Message$ until we get the message ``Onion from $x$ with message $m$ for $r$ routed through ...''. We then now that this message $m$ belongs to the sender whose onion was not $temp'$(because we blocked this onion) and hence, we will pick the guess according to the linking we learned.

\item $\SMO$ for  $C_{P,c^{S}}$:
Analogous to $\PairSML$ for  $C_{P,c^{S}}$, although we do not need to block any $temp'$ as in the simplest attack there is only one communication in both scenarios and hence, this one can be traced.

\item $\PairRML$,$\RMO$, $\MOm$ for  $C_{P,c^{S}}$:
We are allowed to pick corrupted receiver, hence we do this and get the receiver-message linking output from the ideal functionality in the  ``Onion from $x$ with message $m$ for $r$ routed through ...''- message after we used $Deliver\_Message$ whenever possible.

\end{proof}

\paragraph{Summary:}
In case of a corrupted receiver none of the notions is achieved. It is intuitive, that if the receiver is corrupted no confidentiality ($\conf$) is achieved. However, also the (honest) sender is not protected in this case.

In case of a honest receiver, confidentiality ($\conf$) is achieved (even if the adversary does not control any relay). This implies that also the linking between the real message and the sender or receiver is protected and also the set of real messages that are sent cannot be learned, since the adversary cannot learn the real message. However, nothing else is achieved; especially the linking between communicating senders and receivers can be learned.

==> sections/hornet.tex <==
Here we first describe the adapted forward phase of HORNET's~\cite{chen_hornet:_2015} data transmission phase in more detail and then analyze it according to our new properties. 

\subsubsection{More Details to Original Transmission Phase}
HORNET's setup creates forwarding segments $FS$ that store the state of the session. To relieve the relays from storing state while the data transmission phase, those $FS$s are sent in an anonymous header $AHDR$. The $AHDR$ at a certain relay includes its  $FS$ (which in turn contains a symmetric key $s$, the routing information and an expiration time), the blinded $FS$s for other relays and a MAC over the first two. Further, an onion layer in the data transmission includes an unencrypted common header $CHDR$ carrying the $type$ ``data packet'', the maximum allowed length of a path $hops$ and an initialization vector $IV$. $IV$ is used for the layered encryption of the payload of the onion layer and updated with a \ac{PRP} at every hop. 

\subsubsection{Adaption}
As such, the type field of the common header \(\mathrm{CHDR}\) distinguishes between a HORNET setup packet, a forward data packet and a backward data packet.
Algorithm \(4\) in~\cite{chen_hornet:_2015} describes the construction of an anonymous header.
\(\mathrm{CREATE\_AHDR}\) works as this algorithm except that it includes the payload layer \(O_i\) and common header \(CHDR_i\) in the calculation of the MAC \(\gamma_i\) (and therefore has those as additional input).
Specifically, \(\gamma_{l-1} \gets \mathsf{MAC}(h_{\mathsf{MAC}}(s_{l-1});FS_{l-1}||\beta_{l-1}||\underline{O_{l-1}|| \mathrm{CHDR}_{l-1}})\) (line $7$) and \(\gamma_i \gets \mathsf{MAC}(h_{\mathsf{MAC}}(s_i);FS_i||\beta_i||\underline{O_i|| \mathrm{CHDR}_i})\) (line $10$).
%This only works for the forward path, as the sender already knows the payload for to be sent packets.

This implies that the onion-encrypted payloads and common headers must be created before the anonymous header is constructed.
Therefore, the anonymous header must be recreated for every transmitted data packet.
This affects source processing of a data transmission packet by adding an additional step to generate an appropriate \(\mathrm{AHDR}\) before sending \(\{\mathrm{CHDR},\mathrm{AHDR},O_0\}\).


%As the value of the $type$-field is unencrypted, different values of $type$-fields introduce different anonymity sets. Hence,in our analysis honest and trusted parties always choose onions with the same $type$-field, but the adversary is allowed to do attacks based on changing the type field.

\subsubsection{Privacy Proof}
The proof for onion correctness is analogous to the one in~\cite{chen_hornet:_2015}. The proof of  the OS properties for the forward direction follows:

\begin{proof}
The used cryptographic primitives $PRG2$, $PRP$, $ENC$, $DEC$, $MAC$, $h_{PRP}$, $h_{ENC}$, $h_{PRG2}$ are modeled as random oracles.

As we need two arguments multiple times we introduce them first:

\emph{Symmetric key $s$ is a secret:}
The adversary does not know the secret key $SV$ of the honest node. Assume she could extract the symmetric key $s$ from the $FS$. Thus she would be able to calculate $PRP^-{1}(h_{PRP}(SV); FS)$ without knowing $SV$, which contradicts the assumption of a secure PRP and secure hash function. Hence, the adversary cannot know $s$ and only guess it with negligible probability.

\emph{$hops$ and $type$ of $CHDR$ and the length of the payload $|O_i|$ are fixed values:}
As explained above we analyze with the $hops$- and $type$-value fixed. As we analyze the data transmission in forward direction an honest sender picks $type$ to be a data packet and forward direction. Changing it to be a setup packet would only cause setup packet processing and hence doing an integrity check including the $CHDR$ that fails because of the modification except for negligible many cases. 
Changing it from forward to backward  leads to a failure of the MAC as they are calculated over different parts of the onion in both cases and the adversary does not know the shared symmetric keys $s$ used in the MAC for honest nodes. Thus, changing the $type$ field does not give any advantage and we can view the $type$ field to be always fixed.
Changing the $hops$ or the length of the payload is not possible for forward onions as this is protected with the MAC. %It is also not possible for backward onions as there the honest nodes check those against fixed system parameters. 

$\mathbf{\OSSenderNode}$
Recall that $\OSSenderNode$ allows the adversary to decide the inputs to $\FormOnion$ and either returns the resulting onion $O_1$ of this $\FormOnion$ call or a randomly chosen onion $\bar{O}_k$, that only matches the subpath between the honest nodes, together with the processing of $O_1$ after the honest node ($\ProcOnion(O_j)$). Furthermore, it allows oracle use before and after this decision.

\emph{No dependencies between $\FormOnion$:}
We define the game $\OSSenderNode^1$ to be the same as $\OSSenderNode$ except that the adversary has no oracle access before his input decision (skips step 2)). As the creation of onions in HORNET's data transmission phase works independent from earlier creations (except they share some equal input), oracle access before the challenge does not improve the adversary's success in guessing correctly. \todo[inline]{Do we have better arguments for this?}


\emph{No modification:}
We define the game $\OSSenderNode^2$ to be the same as $\OSSenderNode^1$ except that the adversary has no oracle access after his input decision (skips step 7)).
Using the oracle for a new onion $\tilde{O}$ independent of the challenge onion $O$ (which is either $O_1$ or $\bar{O}_k$) resp. of their processing does not help guessing $b$ as the output $\ProcOnion(\tilde{O})$ is then independent from $b$ as well. 
Thus, we only need to look at modifications  of the challenge onion processed until the honest node $O_{+j}:=\ProcOnion^j(O)$.
As any onion layer in the data transmission, $O_{+j}$ consists of three parts $(CHDR, AHDR, o)$.  
In the forward phase all those components are completely secured by a MAC and thus modification is only successful with negligible probability.
Therefore, there cannot be a successful attack on $OS_{p}^1$ that relies on the second oracle and thus any successful attack on $OS_{p}^1$ is also possible for $OS_{p}^2$ in HORNET.

\emph{No linking:}
We define the game $\OSSenderNode^3$ to be $\OSSenderNode^2$ but the second part of the output ($ProcOnion(O_j)=(O_{j+1}, P_{j+1})$) is no longer given to the game adversary. Assume knowing this output helps the adversary to break $\OSSenderNode$. 
As the next hop $P_{j+1}$ is already known to her from her choice of path, the only part of the output that can help her is $O_{j+1}$.
Thus the adversary must be able to link  $O_{j+1}$ to the first output onion layer ($O_1$ resp. $\bar{O}_k$) which differs depending on $b$. Hence, she must be able to link the onion layers  before and after the honest node. 
Onion layers in the data transmission consist of three parts $(CHDR, AHDR, O)$. The first two parts of $CHDR$ include the fixed type and length of the longest path. The remaining part of $CHDR$ is $IV$. The processing at a honest node changes the non-fixed parts: $IV'=PRP^{-1}(h_{PRP}(s); IV)$, $O'=DEC(h_{ENC}(s); IV; O)$ and $AHDR'=\{ \beta |0^c\}\oplus PRG2(h_{PRG2}(s))$. Assume if the adversary can decide on $(IV, AHDR, O)$ she can distinguish any of the new values $(IV',AHDR', O')$ from randomness without knowing $s$. However, this implies that she is able to break the secure $PRP$, $DEC$, $PRG2$ or the hashes, which contradicts the assumption for those primitives.

Thus, no successful attack on $\OSSenderNode^2$ based on the second part of the output ($ProcOnion(O_j)$) can exist for HORNET. Therefore every successful attack on $\OSSenderNode^2$ in HORNET is a successful attack on $\OSSenderNode^3$. Hence, for HORNET $\OSSenderNode^3 \implies \OSSenderNode^2$.


\emph{Onion layer indistinguishable from random ones:}
We define $\OSSenderNode^4$ to be $\OSSenderNode^3$ except that for the output onion layer $(CHDR, AHDR, O)$ the values of $CHDR, AHDR$ and $O$ are chosen randomly from their corresponding spaces, such that the multiple processing of the onion layer results in the same subpath as given by the adversary.
 We show that $\OSSenderNode^4$ is indistinguishable from $\OSSenderNode^3$.
 Assume an adversary that can distinguish the games.
 As the multiple processing of the onion layer results only in expected behavior,  she  must be able to distinguish some of the parts of the onion layer from randomness.
Assume she can distinguish $CHDR$. $CHDR$ contains a fixed $type$ and the fixed number of the longest length of a supported path. As those are fixed they will not be drawn differently as $CHDR$ is drawn randomly.  $IV$ is choosen uniformly at random by the sender in HORNET, if it is the $IV$ for the last relay or calculated as $PRP(h_{PRP}(s); IV')$, which is indistinguishable from randomness as PRP is a random oracle.  So she cannot distinguish $CHDR$.
Assume she can distinguish $AHDR$. $AHDR$ contains $FS, \gamma, \beta$.  $FS, \gamma, \beta$ are indistinguishable from random values as otherwise it would contradict the assumption of the secure $PRP$, $MAC$ or $PRG2$.
Assume she can distinguish $O$ when it is not the onion layer after the last honest node, then she could distinguish the result of a decryption for which she does not know the key.
The result of the decryption is another encrypted onion layer, as it is not the onion layer after the last honest node.
Therefore, she cannot distinguish the decryption result from a randomly drawn value, and also not process it to get the message.

\todo[inline]{I am ignoring that the combination of those parts might be distinguishable..}

In $\OSSenderNode^4$ all the values are drawn the exact same way for both cases of $b$, there cannot be an adversary with any advantage for this game. Because $\OSSenderNode^4\approx \OSSenderNode^3 \implies \OSSenderNode^2 \implies \OSSenderNode^1 \implies \OSSenderNode$, we have proven that any adversary has only negligible advantage in guessing $b$ for $\OSSenderNode$.

$\mathbf{\OSNodeReceiver}$
Recall that $\OSNodeReceiver$ either outputs the processing of the onion build from the adversary's choice ($\ProcOnion(O_j)=(O_{j+1},P_{j+1})$) or the processing from a random onion that matches the end of the path and message of the adversary's choice ($\ProcOnion(\bar{O}_k)=(\bar{O}_{k+1}, P_{j+1})$). Note that the next hop is always the same in those outputs and thus only the onion layers need to be indistinguishable. To show this is analogous to $\OSSenderNode$'s ``Onion layer indistinguishable from random ones'' except that $O$  is chosen randomly from the onion layers that also include the adversary chosen message.


% OLD PROOF
%We adopt the hybrid-game method. First, we con-
%struct a modified game $G_1$ with exactly the same definition, except
%that we require $j = 0$. An adversary who can win $G$ can thus immediately win $G_1$ . On the other hand, because the adversary controls
%nodes$ (n_0 , . . . , n_{j−1})$ $((n_0', . . . , n_{j−1}' ))$ and can thus emulate their
%processing, the adversary can also win game $G$ if he/she can win
%game $G_1$ . Therefore, the adversary can win game $G$ if and only if
%the adversary can win game $G_1$ .
%We create a second game $G_2$ , which is the same as $G_1$ except
%that $F$ $S0$ , $β0$, and $γ0$ are all randomly generated from their corresponding domains. If the adversary can distinguish $G_2$ from $G_1$ ,
%we have:
%1. The adversary can distinguish
%$F S_0 = P RP (hP RP (SV0); R0 ||s0 )$
%from randomness. Then it must be that the adversary is able
%to tell the output of a pseudo-random permutation with a ran-
%dom key $(hP RP (SV0 ))$ from random bits. The probability
%of success for the adversary is negligible.
%2. The adversary can distinguish
%$β0 = P RG(hP RG (SV0 )) XOR {F S1||\gamma_1 ||\beta_1 }$
%from randomness. Then it must be the adversary is able to
%distinguish the output of a secure pseudo-random number
%generator with a random key $(hP RG (SV0 ))$ from random-
%ness. The probability that the adversary succeeds is negligible.
%3. The adversary can distinguish
%$\gamma_0 = M AC(hMAC (SV0 ); \beta_0 )$
%from randomness. Then it must be the adversary is able to
%distinguish the output of $MAC$ with a random key $hMAC (SV0)$
%from randomness. Under our random oracle assumption for
%M AC, the probability of success is negligible.
%Therefore, the adversary cannot distinguish $G_2$ from $G_1$ .
%Lastly, because in $G_2$ , $(F S0 , \gamma_0, \beta_0)$ are all random, the adversary’s advantage is 0.
% Moreover, in our chain of game $G \rightarrow G_1 \rightarrow G_2$ , the adversary can only distinguish a game from its previous
%game with negligible probability. As a result, the adversary’s advantage in game $G$ is negligible.

\end{proof}




==> sections/hornetBackground.tex <==
\label{sec:backgroundSphinx}
One proposal for an \ac{OR} protocol is \emph{HORNET}~\cite{chen_hornet:_2015}. HORNET is proposed as a high-speed, highly scalable anonymity system for the network layer. The attacker is assumed to actively control a fraction of the relays, i.e. at those relays the attacker can replay, redirect and modify packets. It promises that such an adversary cannot link the sender Alice to her message or the receiver Bob even if Bob is compromised.
To achieve this features, HORNET adapts the secure \ac{OR} packet format Sphinx~\cite{danezis_sphinx:_2009}  for the setup phase which enables it to create an anonymous header for routing in the data transmission phase. Multiple cryptographic primitives are used in the construction and processing of packets in both phases. At this point, we only need to highlight some techniques of the data transmission phase. There the packet consists of a common header, which carries an initialization vector and the maximum path length, an anonymous header, which carries the path information, and the data payload, that carries the message. The common header is unencrypted and the maximum path length allows to determine the length of the anonymous header. The  integrity of the anonymous header is protected with a \ac{MAC} at each layer. The payload however is not checked for integrity. Further, the encryption of the payload at every relay is done with a stream cipher and the initialization vector of the common header.


The privacy of HORNET's setup phase is claimed to follow from Sphinx. The privacy of HORNET's data transmission phase is proven following the formal treatment described in~\cite{camenisch2005formal} as it is done for a variety of works like the improved Minx~\cite{shimshock_breaking_2008},  Sphinx~\cite{danezis_sphinx:_2009} and Taranet~\cite{chen_taranet:_2018}.

==> sections/introHornet.tex <==
We have shown that the original properties were not sufficient to achieve the privacy guaranteed by the ideal functionality.
However, there is no immediate connection to the attacks on Sphinx and HORNET, as described in Section \ref{sec:attack}, so far.
%Although we learned that the properties were not sufficient before and we have seen which parts we needed to improve, there is no immediate connection between our insights and the attack on the packet formats and systems in Section \ref{sec:attack}. 

In the following section, we will investigate the connection between the  new security properties and  the attack, first.
We then show that a version of Sphinx that has been improved for performance actually does guarantee the privacy of the ideal functionality and our new properties.
%In the first part of this section, we want to give the connection between the attack and properties. In the second part, we show that a performance-improved version of Sphinx guarantees the privacy of the ideal functionality by proving our new properties.


==> sections/introSystems.tex <==
So far, we learned about the underlying proof strategy and corrected the flaws there. In this section, we consider the ramifications for the proposed systems. %Thereby, we first focus on HORNET and then on the related works.

==> sections/maxPathLength.tex <==
We assume that any layer increases the onion size by at least $1$\,Bit. As our following onion security properties further imply that onions generated within the onion security games have the same size independent of their actual path length, 
We need the onion routing protocol to support a maximum path length $N$ in terms of hops between an honest sender and a receiver.
This allows padding to be applied in order to yield fixed sized onions independent from the $FormOnion$ input.



==> sections/privacyFunctionality.tex <==
We analyze the ideal functionality first against the adversary model for \ac{OR} described in \ref{sec:ORBackground}. Thus, the adversary is especially able to observe controlled links and drop or delay onions on these links. Thereby we will see that all notions, except $\conf$ (confidentiality), are broken due to a simple traffic analysis attack.

\subsubsection{Instantiation of the Framework}\label{sec:frameworkInstance}
As the path $\mathcal{P}$ is an important input to an onion, we model it specified in the auxiliary information of a communication.
The communications, including the auxiliary information, are picked arbitrarily by the adversary in the framework. 
Assumption \ref{as:honestOnPath} however requires at least one honest relay to exist on the path for our analysis.
For this reason, we define the path-modifying adversary class $\pathAdvClass$: It replaces the paths as chosen by the adversary with alternative paths, whenever an honest sender is assumed to construct the onion. 
The replacements are chosen at random from the set of paths with valid length that include at least one common honest relay.%, such that they conform to the maximum path length. 

\subsubsection{Analysis}
Recall, the ideal functionality only outputs the message to the adversary for a corrupted receiver or sender. So, the message is protected if sender and receiver are honest or corrupted users get the same messages in both scenarios (limitation in $\corrStandard{X}$). However, all other notions but confidentiality $\conf$ can be broken as the adversary decides when an onion is forwarded. She hence can decide to only allow one onion to be forwarded and observe its path.
This brings us to Theorem \ref{theo:AnalysisWrongAdv}, which is proven in
 \iflong    % tex currently not used
 Appendix \ref{app:onlyConf}.
 \else
more detail in our extended version~\cite{extendedVersion}.
 \fi


\begin{theorem}\label{theo:AnalysisWrongAdv}
$\originalIdeal$ achieves $\corrStandard{\conf}$ and all those implied by it, but no others (of  \cite{ownFramework}) for $\pathAdvClass$.
\end{theorem}


%In case of corrupted receivers or senders even the message is learned and hence none of the notions achieved.
%In case of an honest receiver and sender, confidentiality ($\conf$) is achieved. 
Note that especially the linking between communicating senders and receivers ($\PairSRL$) and for corrupted receivers the linking between sender and messages ($\SML$) can be learned.
This is neither what \cite{camenisch2005formal} claims, nor what we expect from \ac{OR}, as it is introduced to hide the linking between sender and real message particularly in the case of a corrupted receiver.


==> sections/relatedWork.tex <==
We split the related work into systems analyzing the security of onion routing schemes, work based upon theses analysis results and formal frameworks available for privacy analysis of communication systems.

\paragraph{Secure Onion Routing}
Camenisch et al.~\cite{camenisch2005formal} were the first to model onion routing as an ideal functionality supporting universal composability as well as presenting properties to ease security analysis of onion routing protocols.
Their presented ideal functionality supports universal composability and thus can be used as building block to construct onion routing models and simplify privacy analysis.
Kate et al.~\cite{kate_pairing-based_2010} adapted some of the previous properties and introduced a few new ones.
Backes et al.~\cite{backes_provably_2012} did not use the established properties, but constructed new ones and also presented an universally composable ideal functionality for the more specific Tor model within onion routing.

\paragraph{Usage of OR Properties}
Properties presented by Camenisch are used in a wide variety of later on proposed systems like Sphinx~\cite{}, Minx2~\cite{}, cMix~\cite{} and indirectly within systems building upon these, e.g. HORNET~\cite{} and Taranet~\cite{}.


\paragraph{Privacy Analysis Frameworks}
AnoA~\cite{}, Hevia et al.~\cite{}, Gelernter et al.~\cite{}, Bohli et al.~\cite{}, Kuhn et al.~\cite{}.


==> sections/sessionsAndReply.tex <==
\subsubsection{Reply Channels}
All systems above consider a reply channel, for example to respond to an anonymous sender.
None, however, analyzes the backward phase separately, they (if at all) only show indistinguishability to the forward onions, implying that the same security properties are used for the reply channel.
% and thus use the same properties for it. 
However, our analysis showed that the privacy goals except confidentiality ($\conf$) are only guaranteed for an honest sender. 
In a reply phase this sender is the original receiver, which cannot ultimately be considered honest. 

Thus, proving the properties does not guarantee the anonymity of the initial sender for a corrupted receiver in the reply phase. 
We conjecture that an adapted ideal functionality and properties will have to be defined for the privacy and security of a reply phase, in future.

\subsubsection{Sessions}
HORNET and TARANET additionally introduce sessions.
Their data transmission phase reuses the same path and header to efficiently send multiple onions. 

The ideal functionality does not cover sessions.
As for a corrupted relay it is always possible to link onions of the same session, neither the properties, nor ultimately the ideal functionality can be shown in this case.
%In such an setting, the properties and ideal functionality cannot be shown as for corrupted relays it is always possible to link onions to the same session, which is not possible in the ideal functionality. %Translated to the onion security properties the adversary can exploit creating (or guessing) another onion for the same session and input it to the oracle\todo{true?}. 
We conjecture, again, that an adapted ideal functionality and  the corresponding properties will have to be defined, in future. 

==> sections/sphinx.tex <==
Sphinx~\cite{danezis_sphinx:_2009}\label{sec:sphinx}

Sphinx uses a further input to $\FormOnion$ a bit $f$ that decides whether the onion is a forward or a reply message. As the receiver learns this bit, we require it to be fixed  for $\OSNodeReceiver$ (like the message). For $\OSSenderNode$ and $\OSNodeNode$ it is chosen randomly for the replacing onion.


\todo[inline]{Which naming of variables to follow here?}
\begin{theorem}[$\OSSenderNode$]\label{thm:OSSN}
  A polynomially restricted adversary has only negligible advantage winning $\OSSenderNode$. % \textbf{G}\(^{\equiv P}\).
\end{theorem}

\begin{proof}
$\OSSenderNode$ returns the first onion layer \(((\alpha_{1}^{b} , \beta_{1}^{b} , \gamma_{1}^{b} ), \delta_{1}^{b})\) according to $b$ and the onion layer after the honest node for $b=0$ \((({\alpha_{j+1}^{0}}' , {\beta_{j+1}^0}' , {\gamma_{j+1}^0}' ), {\delta_{j+1}^0}')\).
We show two things: (1) The onion layer after the honest node does not allow any conclusion about the before the honest node.
(2) The first onion layer that is output cannot be distinguished from one where the parts of the onion are chosen randomly.
Notice that once we have shown (1), it is clear that the second output \((({\alpha_{j+1}^{0}}' , {\beta_{j+1}^0}' , {\gamma_{j+1}^0}' ), {\delta_{j+1}^0}')\) does not help in distinguishing $b$. With (2) we further know, that also the first output  \(((\alpha_{1}^{b} , \beta_{1}^{b} , \gamma_{1}^{b} ), \delta_{1}^{b})\) cannot be distinguished from randomness and hence  we know that the adversary's advantage in the original game \(\OSSenderNode\) is negligible, as required.

(1) Given an onion layer \(O_{j+1}=(({\alpha_{j+1}} , {\beta_{j+1}} , {\gamma_{j+1}} ), {\delta_{j+1}})\), consider the following game: The challenger chooses a bit $b$ and if $b=0$ an onion layer \(O_j=(({\alpha_{j}} , {\beta_{j}} , {\gamma_{j}} ), {\delta_{j}})\) with $\ProcOnion(f(O_j))= (P_{j+1}, O_{j+1} )$ and if $b=1$ an onion layer \(O_j\) with $\ProcOnion(f(O_j))= (P_{j+1}, O_{j+1}' )$. We show the adversary cannot guess $b$ with a non-negligible advantage.

The only way to decide whether $O_{j+1}$ belongs to $f(O_j)$ is to find a connection in some of their parts \((({\alpha_{j+1}} , {\beta_{j+1}} , {\gamma_{j+1}} ), {\delta_{j+1}})\). 
Assume the adversary could based on knowing $\alpha_j$ and picking a PPT modification function ${f}$ distinguish a correctly from $\mathcal{f}(\alpha_j)$ generated $\alpha_{j+1}$ from a randomly chosen $\alpha_{j+1}'$. Thus, she could solve the decisional Diffie-Hellman problem using ${f}$  (distinguish ???...)
\todo[inline]{Can't reduce it to DH problem...as $(g^a, g^b, g^{ab})$,$(g^a, g^b, g^c)$ with $a,b,c$ independently chosen...
we would have $g^{ab}= ( {f}(g^{xb_0..b_{j-1}}))^{h_b( {f}(\alpha_{j}), s_j)}=^? g^{{f}'(x)b_0..b_{j}'}$ However, I do pick $a$ and $b$ one always includes function $f$ (or deduced function $f'$, if this is even possible), so I cannot solve it for $a$ and $b$ chosen  randomly}

Assume the adversary could link them based on $\beta$. $\beta_{j+1}$ is the XOR of $\beta_{j}$ with the result of the PRG with the hashed secret $s_j$. As the adversary does not know this secret shared between the honest sender and honest relay and it never uses the same stream multiple times, she has no advantage distinguishing $\beta_{j+1}$ from a random string. Even if she modifies $\beta$ this is the same as a XOR with another result of the PRG and hence does not help her distinguish the $\beta_{j+1}$. 

Assume the adversary could link them based on $\gamma$. $\gamma_{j+1}$ is the MAC over $\beta$ with the hash of the shared secret, that can be modeled as PRF, the adversary cannot distinguish it from a random other $\gamma$.

Assume the adversary could link them based on $\delta$. $\delta_{j+1}=\Pi^-1(h_\Pi (s_j), \delta_j)$. As $\Pi$ is a PRP the adversary cannot distinguish it from a random other $\delta$.

(2) 
We use the usual method of hybrid games.

\textbf{Random shared secret $s_0$ to randomize \(\beta_1\) and \(\gamma_1\).}
Game  \textbf{G}\(^{\OSSenderNode}_1\) is the same as \(\OSSenderNode\), except for selecting \(s_0\) uniformly at random from \(\mathcal{G}^*\), as opposed to being calculated as \(s_0 = {y}_{n_0}^{x}\).
An adversary that can distinguish game \(\OSSenderNode\) from \textbf{G}\(^{\OSSenderNode}_1\) can distinguish \(({y}_{n_0} , \alpha_0 = g^{x} , s_0 = {y}_{n_0}^x )\) from \((y_{n_0} , \alpha_0 , z)\) for random \(z \xleftarrow{R} G^*\) , thus solving the DDH problem in \(G^*\) , contrary to our choice of \(G^*\).

Here it is important that the adversary should not be allowed to query \(N\) with the challenge \((\alpha_1^b , \beta_1^b , \gamma_1^b )\) header, since \(N\) would not be able to process it.
That \(\gamma\) must be a MAC on \(\beta\) with key \(h_\mu(\alpha_1^{x_{n_0}} )\) ensures that \((\alpha_1 , \beta, \gamma) \neq (\alpha_1 , \beta_1 , \gamma_1 )\) will be rejected by \(N\) except with negligible probability.
If any \((\alpha, \beta, \gamma)\) is submitted to \(N\) with \(\alpha \neq \alpha_1\) such that \(N\) successfully processes the message, then the success of the MAC ensures that, again except with negligible probability, the adversary knew the MAC key \(h_\mu(\alpha_1^{x_{n_0}} )\).
Since \(h_\mu\) is a random oracle, the adversary must have queried it with \(\alpha_1^{x_{n_0}}\).
But if the adversary knows that last value, she can process the message just as well as \(N\) can, and the ability to query \(N\) does not help her.

\textbf{select \(\beta_1,\gamma_1\) at random.}
Game \textbf{G}\(^{\OSSenderNode}_2\) is the same as \textbf{G}\(^{\OSSenderNode}_1\) except that \(\beta_1\) and \( \gamma_1\) are selected uniformly at random from their respective domains.
If the adversary can distinguish games \textbf{G}\(^{\OSSenderNode}_2\) and \textbf{G}\(^{\OSSenderNode}_1\) , then she can distinguish (with less work than \(2^\kappa\) ) the output of \(\rho\) with a random input from a random string, or \(\mu\) with a random key from a random function, which she can do with only negligible probability, by our choice of \(\rho\) and \(\mu\).

\textbf{select \(\delta_1\) at random.}
Game \textbf{G}\(^{\OSSenderNode}_3\) is the same as \textbf{G}\(^{\OSSenderNode}_2\) except that \(\delta_1\) is selected uniformly at random from its respective domain.
If the adversary can distinguish games \textbf{G}\(^{\OSSenderNode}_3\) and \textbf{G}\(^{\OSSenderNode}_2\) , then she can distinguish (with less work than \(2^\kappa\) ) the output of \(\pi\) with a random key \((h_\pi(s_0)\) -- with \(s_0\) being the randomly selected value from game \textbf{G}\(^{\OSSenderNode}_1\) -- in the case of forward messages, or \(\tilde{k}\) \todo{check if $f$ needs to be fixed} in the case of reply messages) from a random permutation, which she can do with only negligible probability, by our choice of \(\pi\).

\textbf{remove inner dependency of \(\alpha_2\) on \(\alpha_1\).}
Game  \textbf{G}\(^{\OSSenderNode}_4\) is the same as \textbf{G}\(^{\OSSenderNode}_3\), except for replacing \(h_b(\cdot,\cdot)\) with a random function \(h_r()\).
An adversary that can distinguish \textbf{G}\(^{\OSSenderNode}_4\) from  \textbf{G}\(^{\OSSenderNode}_3\), thus \(\alpha_2 = {\alpha_1}^{h_b(\alpha_1,s_0)}\) from \({\alpha'}_2 = {\alpha_1}^{h_r()}\) can distinguish the output of \(h_b\) from a random function, contrary to our choice of \(h_b\).

\textbf{select \(\alpha_1\) at random.}
Game  \textbf{G}\(^{\OSSenderNode}_5\) is the same as \textbf{G}\(^{\OSSenderNode}_4\), except for selecting \(\alpha_1\) uniformly at random from their respective domain.
Selecting a random \(\alpha_1\) is equivalent to selecting a different \(x' \neq x\) with \(\alpha_1 = g^{x'}\).
Due to \(G\) being a cyclic group of prime order \(q\), exponentiation of an element \(\alpha_1 \in G^*\) with a random value \(r = h_r()\) (\(r \in \mathbb{Z}_q^*\)) generates pseudo random elements in \(G^*\).
Thus, \(\alpha_2\) could have been generated from the random \(\alpha_1\)\todo[inline]{\(|G^*|-1 = |\mathbb{Z}_q^*|\) is that true? if so: is it an issue. Probably not, as \(1\) is negligible in \(\kappa\). \(q \approx 2^{2\kappa}\)} and an adversary that can distinguish the random \(\alpha_1\) from random elements in \(G^*\) can be used to distinguish \(h_r\) contrary to the choice of \(h_r\).

In game \textbf{G}\(^{\OSSenderNode}_5\), since \(\alpha_1,\beta_1,\gamma_1,\delta_1\) are all random, they cannot be linked to \(\alpha_{j+1},\beta_{j+1},\gamma_{j+1},\delta_{j+1}\).
Since \(\alpha_1,\beta_1,\gamma_1,\delta_1\) are all independent of \(b\) and \(\alpha_{j+1},\beta_{j+1},\gamma_{j+1},\delta_{j+1}\) is identical (independent of \(b\)), it is clear the adversary's advantage is \(0\).
Since each game is indistinguishable from the one before to the adversary, except with negligible probability, we see that the adversary's advantage in the original game \(\OSSenderNode\) is negligible, as required.
\end{proof}

$\OSNodeNode, \OSNodeReceiver$ are argued similarly.

==> sections/sphinxBackground.tex <==
\label{sec:backgroundSphinx}
One proposal for an \ac{OR} format is Sphinx~\cite{danezis_sphinx:_2009}. Sphinx main features are to provide bitwise unlinkability between onion layers before and after an honest node, hiding the number of hops an onion already travelled, indistinguishability of reply and normal onions, resistance against all active tagging attacks that target learning the destination or message, and space efficiency.
Thereby the attacker model assumes an active adversary that controls all links, i.e. can observe, modify, drop and insert onions on them. Further, some of the relays are in adversarial control and especially a corrupted receiver cannot learn the originator of the message for her. However, attacks on traffic analysis, flooding or denial of service are excluded, but tagging attacks, i.e. the adversary modifies the onion before reinjecting it, are allowed .
To achieve the features against this adversary, Sphinx defines its onion layers to consist of a header, which contains the path, and a payload, which contains the message. Multiple cryptographic primitives are used to construct and process them. At this point, we only want to highlight that the integrity of the header is protected with a \ac{MAC} at each layer, but no such protection for the payload at each layer exists. Tampering with the payload is only recognized at the receiver. Further, the processing of the payload is done with a \ac{PRP}.

The privacy of Sphinx is proven following the formal treatment described in~\cite{camenisch2005formal} as it is done in a variety of systems like Minx2~\cite{shimshock_breaking_2008} , HORNET~\cite{chen_hornet:_2015} and Taranet~\cite{chen_taranet:_2018}. The latter two even base their systems setup phase on Sphinx.

==> sections/sphinxProofFails.tex <==
From Section \ref{sec:IdealAnalysisConsequences} we know that Sphinx as in~\cite{danezis_sphinx:_2009}  does not realize the ideal functionality. Therefore, the attack on Sphinx from Section \ref{sec:attackSphinx} has to translate to an attack on our properties (or else we have a contradiction). We can give the following related attack on $\OSSenderNode$: The adversary does her choices randomly, but valid and stores them. Then the adversary receives the two challenge onion layers ($O_1,O_{j+1}$) and processes $O_1$ until $O_j$. Then the adversary modifies only the payload of $O_j$ and hands this modified onion layer to the oracle to receive its processing. Now, the adversary can keep processing this onion layer and learn the path after the honest relay. She thus can compare it with her input choice for $\FormOnion$ and if it matches she guesses that the original onion was given to her. Otherwise, she guesses that she received the fake. As Sphinx choice of path only depends on the header and not the payload, the modified onion takes the same path and thus the adversary wins, unless a fake onion with the exact same path was chosen, which only happens with a small probability.

There is no connection between our changes in the properties and the Sphinx attack as another flaw in argumentation is the reason for it: In Sphinx's analysis this attack was excluded by an adaption in the oracle after the challenge onion was given to the adversary. There the oracle allowed only non duplicates to the challenge onion as input.
 Since Sphinx's duplicate check works only on the header, giving an onion layer with only modified payload to the oracle as in our attack is no longer allowed. 
 The adaption seems reasonable if one thinks about the oracle after the challenge as new onions the adversary creates and sends to the honest relay after the challenge onion was already processed by it. However, this oracle is needed to exclude all modification attacks that in the real world modify the challenge onion before it was processed by the honest relay as well.
This adaptation thus weakens the properties, such that they no longer imply realizing the ideal functionality. In \ref{longVersion}, we show a way to compensate this weakening with a third property. This allows to prove protocols with special duplicate checks, for which the properties presented here cannot be shown, to be proven secure.
  
The same flaw in argumentation and thus a similar attack exist in the extension to the protocol in~\cite{camenisch2005formal} (Sec. 4.2).

==> sections/unused/extensionLeaksNotMore.tex <==

\begin{theorem}
  The extended protocol \(\PiOI\) leaks not more information to an adversary \(\mathcal{A}\) than the underlying protocol \(\Pi\).
\end{theorem}

We show this theorem by contradiction.
\todo[inline]{Some active attacks are missing: modified onion is not processed anymore, hence attacker might additionally learn that an onion is modified (or observe the dropping itself (maybe multiple times; always one hop further as it is able to modify a ``little'' and thus track the path a hop further))}

\begin{proof}
  The proof is split in a \textbf{1)} passive case, where the adversary observes all links and performs processing on corrupted nodes and an active \textbf{2)} case where the adversary manipulates an onion for further information gain.

  \textbf{1)}
  Assume that an adversary learns more than from protocol \(\Pi\).
  The beginning of any onion layer \(O_i'\) generated by \(\FormOnionOI\) is identical to the onion layer \(O_i\) generated by \(\mathrm{FormOnion}\) under identical input (given the same randomness in probabilistic algorithms).
 % They are actually identical given the same randomness as input, as the same algorithm \(\mathrm{FormOnion}\) is used in both protocols.
  The additional knowledge must therefore come from the extension appended by \(\FormOnionOI\).
  It cannot be the length as \(\FormOnionOI\) increases the length of onion layers only by a fixed value compared to \(\mathrm{FormOnion}\) with the same input.

  At the packet level, the extension is a list of \(N\) blocks, consisting of one of the following elements.
  \begin{itemize}
    \item random elements from the asymmetric ciphertext space \(d_i \in \mathcal{C}_{asym}\), as drawn by \(\FormOnionOI\)
    \item encryptions of keys and tags using a semantically secure asymmetric encryption scheme
    \item encryptions in the space of asymmetric ciphertexts using an IND-CCA2 secure symmetric encryption scheme
    \item pseudorandom values generated by a pseudorandom generator from the asymmetric ciphertext space based on key \(KDF(P_i,k_i)\)
  \end{itemize}
  By the security properties of any of these algorithms, the generated blocks cannot be distinguished from random values within the same space and thus leak no additional information.

  The additional knowledge of the adversary must therefore stem from processing the extension.
  A router decrypts the first block using its own asymmetric decryption key.
  It finds a random ephemeral, symmetric key \(k_i\) and a tag \(t_i\).
  The key is random and thus yields no additional information to the adversary.
  The tag is generated by a MACning function that is a pseudo random function and thus is indistinguishable from a random number.
  
  Further, the key is used to symmetrically decode all other blocks received at that router in the extension.
  By construction, the decryptions will either \textbf{a)} yield a pseudorandom number, as the original value was a pseudorandom number, \textbf{b)} the asymmetrically encrypted next block for router \(P_{i+1}\), or \textbf{c)} a symmetrically encrypted block containing an asymmetrically encrypted block for routers further down the path.
  The pseudorandom decryption (\textbf{a)}) does not depend on any input given to \(\FormOnionOI\), except for the number of decryptions, which reflects the current layer position.
  However, it is not possible to extract how many decryptions under different random keys were already performed upon a given ciphertext.
  By the security properties of the symmetric, as well as asymmetric encryption scheme, no information can be extracted from cases \textbf{b)} and \textbf{c)}.
  Further, the tag \(t_i\) authenticates onion layer \(O_{i+1}\) as well as extension blocks using key \(k_i\).
  All input necessary for the creation of tag \(t_i\) is known to the adversary and already argued above to not leak any information, thus \(t_i\) cannot leak any new information.
  %Further, as the message \(m\) that was input to the \(\FormOnionOI\) algorithm is only used as part of an onion \(O_i'\) for creation of tag \(t_i\) and due to the use of a secure MAC system, the adversary does not learn anything about \(m\) by learning any tag \(t_i\).

  As the adversary did not gain any knowledge from the values found, she must have learned something by comparing the extension before and after an honest router.
  A malicious sender already knows all onion layers and can trivially link onions that an honest router receives and sends.
  This is independent from our extension and due to the system model.
  Therefore, we analyze the case of an honest sender.
  Linking onions across an honest router cannot be done just by passively examining the extension, as the honest router processes all blocks and derives pseudo-random blocks indistinguishable to random values due to the properties of the used cryptographic primitives.
  It further adds a pseudorandom block that cannot be predicted, as key \(k_i\) of the honest router \(P_i\) is not known given an honest sender.
  By the same argument, the decryptions of all other blocks cannot be linked (predicted), as they are processed using \(k_i\).
 % A malicious sender can predict these values, but knows them anyway, as she created them in the first place. %Malicious sender excluded before..

  \textbf{2)}
  As the adversary did not learn anything passively, it must have used an active attack to modify the onion.
  Hence, the  linking is based on changing  (\emph{tagging}) the original onion or appended extension before an honest router and recognizing it later.
  However, any change to the extension \(ext_i\) or original onion \(O_i\) will invalidate the contained tag \(t_i\) checked by the honest router \(P_i\), as the tag includes all remaining blocks and the processed onion \(O_{i+1}\).
  Thus, the honest router will discard any manipulated onion.
  
  It follows that the adversary also cannot learn anything by actively modifying onions or extensions.
  This contradicts the assumption that \(\mathcal{A}\) learns more from \(\PiOI\) compared to running \(\Pi\).
\end{proof}

%Note that an adversary might learn, in case the encapsulated tag is wrong, that a non-colluding adversary controlled the router before him or that a malicious sender did not correctly generate the onion.
%However, this additional knowledge does not help him to break any privacy goal. 

==> sections/unused/newOnionSecurityDuplicates.tex <==
Some protocols use a duplicate check different than checking for bitidentical onions. Sphinx for example declares all onions whose header is equal as duplicates. For some of these protocols the afore given property $\OSSenderNode$ from Definition \ref{def:OSSenderNode} is trivially broken. Thus we adapt $\OSSenderNode$ for duplicates. However, to still be strong enough for the privacy of the ideal functionality, we need to add another property that takes care of modifications and was included in $\OSSenderNode$ before. $\OSNodeReceiver$ can stay as it is.

\subsubsection{$\OSSenderNode$ with other Duplicate Filters}


\paragraph{Duplicates (Step 7)} A protocol that defines duplicates different than bit-identical onions (e.g. Sphinx only checks the header as duplicate check), trivially fails $\OSSenderNode$ from Definition \ref{def:OSSenderNode}: the adversary can call the oracle after the challenge (Step 7) with a duplicate of the challenge onion to learn the next hop and hence win the game. In reality however, such an onion is not processed after the challenge onion already was. Thus, we need to adjust the oracle use: only onions that are no duplicates of the challenge onion are allowed as oracle input. Therefore, we use  $\duplicate$ as the function that returns true for two onions, iff the two onions are considered duplicates by the check of the protocol. 

Thus, the adapted property is defined as: 

\begin{definition}[$\OSSenderNode$ (Duplicate Version)]\footnotesize \label{def:OSSenderNodeDupl}
\begin{enumerate}
\item - 6) as  Definition \ref{def:OSSenderNode}
\addtocounter{enumi}{5}
\item The adversary may submit any number of onions $O_i$, $O_i \noduplicate O_j$, $O_i \noduplicate \bar{O}_j$ of his choice to the challenger.  The challenger sends the output of $\mathrm{ProcOnion}(SK, O_i , P )$ to the adversary.
\item The adversary produces guess $b'$ .
\end{enumerate}
\end{definition}


\subsubsection{Modification $\OSMod$}
So far, we did replace the onions and assured that no linking exists and nothing from the onion can be learned as long as the adversary behaves honest-but-curious. However, the adversary can also modify onions instead of processing or forwarding them as the protocol requires. Thus, this property requires that the results of an honest node processing a modified original onion and a modified replaced onion are indistinguishable for the adversary. 

\begin{definition}[$\OSMod$]\footnotesize \label{def:OSMod}
\begin{enumerate}
\item  - 2) As in Definition \ref{def:OSSenderNode}
\addtocounter{enumi}{1}
\item As in Definition \ref{def:OSSenderNode} but the adversary additionally submits a modification function $f$ that does not return the identical, but a duplicated onion for any input.
\item - 5) As in Definition \ref{def:OSSenderNode}
\addtocounter{enumi}{1}
  \item
	\begin{itemize}
		\item If $b = 0$, the challenger gives $O_1, \ProcOnion(f(O_{j}))$ to the adversary
		\item Otherwise, the challenger gives $\bar{O}_k, \ProcOnion(f(\bar{O}_{k+j}))$ to the adversary
	\end{itemize}
\item The adversary may submit any number of onions $O_i \noduplicate f(O_j)$ if $b=0$ (resp. $O_i \noduplicate f(O_{k+j})$ if $b=1$) of his choice to the challenger.  The challenger sends the output of $\mathrm{ProcOnion}(SK, O_i , P )$ to the adversary.
\item The adversary  produces guess $b'$ .
\end{enumerate}
\end{definition}

Note that every adversary to $\OSSenderNode$ from Definition \ref{def:OSSenderNode} can already generate this observations: As the modification function $f$ returns a different onion than the challenge onion, the adversary can observe the processing of the modified challenge onion as well. Further, the first part of the output in $\OSMod$ is chosen in the same way as in  $\OSSenderNode$ from Definition \ref{def:OSSenderNode}.

We summarize the different outputs of the properties with special duplicate checks in Fig.~\ref{fig:OSOutputsMod}.
\begin{figure}[htb]
  \centering
  \includegraphics[width=0.48\textwidth]{Images/OSOutputsMod.pdf}
  \caption{Summary of different outputs for special duplicates definition}
  \label{fig:OSOutputsMod}
\end{figure}

==> sections/unused/problemBackward.tex <==
\paragraph*{Backward direction HORNET data transmission}

We show the properties under special duplicate detection. Therefore, the oracle in $\OSSenderNode$ does not give answers for duplicates of the challenge onion. However, we additionally have to prove $\OSMod$

To simplify the analysis, we further restrict the protocol to only except one maximum path length (~\cite{chen_hornet:_2015} suggests 7 for most cases) and one fixed length of the payload on the backward path. Processing honest routers drop onions with different values. If flexibility in those values is needed they can be added to the common header, but then this part of the header needs to be integrity protected on the backwards path as well.

With this the points \emph{Symmetric key $s$ is a secret}, \emph{$hops$ and $type$ of $CHDR$ and the length of the payload $|O_i|$ are fixed values}, \emph{No dependencies between $\FormOnion$}, \emph{No linking} and \emph{Onion layer indistinguishable from random ones}  hold similar to the argumentation before.

The backward phase is slightly different for \emph{No modification}: We can ignore the $type$ and $hops$ field of $CHDR$ as argued before.
As onions only differing in $IV$  of $CHDR$ and $o$ are not seen as duplicates they cannot be used in the oracle. $AHDR$ is protected by a MAC and thus modification is only successful with negligible probability. Thus, only with negligible probability a modification of the challenge onion returns an answer from the oracle.

Additionally, we need to prove $\OSMod$. Recall that $\OSMod$ allows the adversary to decide the inputs to $\FormOnion$ and either returns the resulting onion $O_1$ of this $\FormOnion$ call or a randomly chosen onion $\bar{O}_k$, that only matches the subpath between the honest nodes, together with the processing of a modification of those onions that results in a duplicate ($\ProcOnion(f(O_j))$ or $\ProcOnion(f(\bar{O}_{k+j-1}))$).  

We argue that the second part of the output does not help distinguishing $b$ and thus the challenge reduces to the first part, which we know is indistinguishable from the argument for $\OSSenderNode$. Note that we do not have to look at the oracles here, as the argumentation as for $\OSSenderNode$ applies.

As $f$ needs to result in a duplicate only  $IV$ of $CHDR$ and $o$ can be changed. As they are only used in the decryption with the adversary unknown symmetric key $s$ ($IV$ as initialization vector, $o$ as ciphertext), changing the ciphertext and initialization vector going into to honest node thus only results in a random bitstring of the length of the payload. This result is the same in both cases as \(DEC\) is a random oracle. Thus, the second output does not help to guess $b$.

==> sections/unused/proofImplyIdeal.tex <==
\label{app:proofImplyIdeal}
\todo[inline]{IS THIS USED?}
We will show that the outputs of any real world protocol $\Pi_0$ (which is satisfying our properties) and attack $\mathcal{A}_0$ on it are indistinguishable from the outputs of the ideal protocol $\mathcal{F}_{Onion}$ and a new constructed attack $\mathcal{S}$, given identical inputs. This implies (as the environment only gets outputs of the protocol and the attacker) that $\Pi_0$ UC-realizes $\mathcal{F}_{Onion}$.

In accordance with the ideal functionality of~\cite{camenisch2005formal}, we need a machine that interacts with the environment and the adversary on behalf of the honest parties and therefore invokes the real world protocol. As the behavior of this machine is never changed, we only argue about the protocol running inside the machine and the adversary. \todo{okay?}

We show the indistinguishability in the outputs as a standard hybrid argument in a sequence of  hybrid protocols and attacks. Therefore, we use two main steps. In the first we show indistinguishability between the original protocol and one where onion layers between honest nodes are replaced with random onion layers (that match the path between the honest nodes and message, if it is observable for the adversary). In the second we show indistinguishablity between using random onion layers and randomly drawn IDs.
In the first step we argue the replacement for onion layers in three parts: first the replacement between an honest sender and the first honest relay, then between any honest relay and the next honest node (relay or receiver) and finally between the last honest node and corrupted receivers. In the second step we argue the replacement in three parts: between honest nodes, between last honest node and receiver and for the case that there is no honest node. \\

\paragraph*{Replacing with Random Onion Layers} We replace the original onion layers $O_i$ with random ones $O_i^R$ that take the same path between the honest nodes. The attacks $A_0',A_0'' A_1,A_2, A_3$ are always the same as $A_0$ except that the corresponding replacement $O_i^R$ instead of the original onion layer $O_i$ is  used (e.g. dropped, modified, delayed or replaced).\\


$\boldsymbol{\Pi_0},\boldsymbol{\mathcal{A}_0}$: Any real world protocol $\Pi_0$ that is generated from secure  $FormOnion$ and $ProcOnion$ as described above and fits the interface to the environment and any real world attack $\mathcal{A}_0$ on it. To fit the interface of the environment the real world protocol\footnote{Technically, this might already be an abstraction of the real protocol, in which e.g. some outputs that do not help the adversary to learn more than on the abstraction like debug outputs are removed.} has to output the onion layer before each honest node to the environment and wait for the notification of the environment that the onion layer was forwarded to the honest node before processing it.
% For the interacts with the UC-environment and the adversary on behalf of the honest parties. Thereby it gives the onion layers for honest parties to the environment and waits for the environment to determine when the onion layer is forwarded.

$\boldsymbol{\Pi_0'},\boldsymbol{\mathcal{A}_0'}$: protocol $\Pi_0'$ behaves like $\Pi_0$ except that it only returns negligible information to the adversary for any message sent to an honest node that is no onion layer.  

\textbf{Indistinguishability 0 and 0':} 
Because of our assumption~\ref{ass:neglInfoOnInvalidInput} the output of protocol \(\Pi_0\) reveals at most negligible information to the adversary for any message that is not allowed to be sent by the adversary in $\Pi_0'$. Hence, the adversary cannot learn more than negligible information from any such message.  If an environment can distinguish the output of $\mathcal{A}_0$ from $\mathcal{A}_0'$ it can be used to break the assumption~\ref{ass:neglInfoOnInvalidInput}. 

$\boldsymbol{\Pi_0''},\boldsymbol{\mathcal{A}_0''}$\footnote{This is no real world protocol.} : protocol $\Pi_0''$ behaves like $\Pi_0'$ except that any node retrieves the processing of onions from a central storage instead of computing it itself.  

\textbf{Indistinguishability 0' and 0'':} 
We only change how the result of ProcOnion is obtained, but the obtained result is still the same. Hence, no output is changed. \\

We now (in \(\Pi_1, \mathcal{A}_1\)) replace the onion layers between the honest sender and the first honest relay\footnote{Notice this might also be the receiver.} for a randomly chosen communication. Afterwards (in \(\Pi_1^*,\mathcal{A}_1^* \)) we repeat this step for all remaining communications. %As a result, within \(\Pi_1^*,\mathcal{A}_1^* \), the first subpath (honest sender to first honest relay) is replaced with random onion layers using the same subpath, for all communications.\todo{the last sentence just repeats the sentence before.}

$\boldsymbol{\Pi_1},\boldsymbol{\mathcal{A}_1}$: Hybrid protocol $\Pi_1$ behaves as $\Pi_0''$, except that for one communication it replaces the onion layers $O_i$ between an honest sender and the first honest relay with the onion layers $O_i^R$ belonging to this subpath for an onion randomly chosen from the set of all valid onions that use the same subpath between the honest nodes. 
This includes that the sender sends the first replacement onion layer $O_1^R$ and that the last replacement onion layer ${O_j^R}$ at the first honest relay $P_j$ results in the next original onion layer $O_{j+1}$ that would be send in the original protocol $\Pi$ (resp. $f({O_j^R})$ results in $\ProcOnion(f(O_{j}))$ for the modification function $f$ used by $\mathcal{A}_0$\todo{we need this to map it to $O_{SN}$, now the central storage in $\Pi_1$ depends on $\mathcal{A}_0$. Is this ok? }). The central storage is adapted to reflect this accordingly. %\footnote{This might be a correct layer of the original onion or the result of the processing of a modified version of the correct layer before the honest node, if the adversary did modify the onion as part of an active attack}. 

\textbf{Indistinguishability 0 and 1:}
If there exists an distinguisher $\mathcal{D}$ that can distinguish outputs of $\Pi_0'', \mathcal{A}_0$ from $\Pi_1, \mathcal{A}_0$, it can be used to construct an attack $\mathcal{A}$ on $\OSSenderNode$  in the following way:

$\mathcal{A}$ uses the same communications as $\mathcal{A}_0$ for $b=0$ of $\OSSenderNode$. Modifications that $\mathcal{A}_0$ does to any of the onion layers before the honest node  either result in a path that still comes across the honest node or not. If the path does not include the honest node, $\mathcal{A}$ knows all the keys used for processing this onion and can simulate its processing till at the receiver. 
Otherwise (the path includes the honest node), the modification function of $\mathcal{A}_0$ is used \todo{We don't use $\mathcal{A}_0$ as blackbox.. is this okay?} by $\mathcal{A}$ and in $\OSSenderNode$ the modified onion is given as input to the honest node. 
For $b=1$ the challenger will pick an onion with a random message and path, except for the part of the path between the honest sender and first honest relay. $\mathcal{A}$ receives the first onion and the onion after the honest node from the challenger. $\mathcal{A}$ executes $\mathcal{A}_0$ except that it replaces the observing of onion layers with the onion layers received from the challenger (and uses ProcOnion and its knowledge about the modifications on corrupted nodes, to generate the other onion layers that the challenger did not directly return, if needed). 
%\todo[inline]{If $\mathcal{A}_0$ is an adaptive attack, $\mathcal{A}$ uses multiple challenges to allow for adaptivity.}\todo{do we actually need this if we exchange one onion layer subpath each time?} 
The resulting outputs of $\mathcal{A}_0$ are given to the distinguisher $\mathcal{D}$, which returns a bit, that $\mathcal{A}$ uses as its guess $b'$.

Clearly, in the scenario for $b=0$, the original onion layers are used and the execution of $\mathcal{A}_0$ equals the one with $\Pi_0$ being used; in the scenario for $b=1$ the onion layers on the subpath until the honest node are replaced with random onion layers, which equals the execution of $\mathcal{A}_0$ for $\Pi_1$. Hence, $\mathcal{A}$ does have the same success breaking $\OSSenderNode$ as the distinguisher $\mathcal{D}$ has distinguishing the protocols.

All the other communications that $\mathcal{A}_0$ needs (e.g. inserted itself) can be simulated by the use of $\ProcOnion$ for the known keys and the use of available oracles\footnote{The oracles are only restricted to not return output for duplicate onions just as the original protocol would not process them.}.\todo{better?}%, which would either lead to breaking \(\OSSenderNode\) or does only provide negligible gain. \todo{true? better?}

$\boldsymbol{\Pi_1^*},\boldsymbol{\mathcal{A}_1^*}$: Replace onion layers on one subpath from honest sender to the first honest relay (where they have not been replaced before) with random layers.

\textbf{Indistinguishability $\boldsymbol{1}$ and $\boldsymbol{1^*}$:} Analogous above. Apply argumentation of indistinguishability ($0\rightarrow 1$) for every newly replaced subpath.\footnote{Technically, we need the onion layers as used in $\Pi_1$ (with replaced onion layers between two honest nodes) in this case. Hence, it is a slightly different game than $\OSSenderNode$: one where the challenger outputs not the real onion layers between those two honest nodes for the chosen communication, but randomly chosen ones with the same path. However, as this further obscures the onions, it is harder to break than the real $\OSSenderNode$ and hence implied by it.}\\

Analogous to the first part, we now (in \(\Pi_2, \mathcal{A}_2\)) replace the onion layers between any honest relay and the next honest node (relay or receiver) for a randomly chosen communication \todo[inline]{(as it would be done without any modification of the adversary)or (this might be the processing of an onion layer that the adversary modified)?}. Afterwards (in \(\Pi_2^*,\mathcal{A}_2^* \)) we repeat this step, but always pick a communication in which the onion layers between the honest relay and the next honest node have not been replaced before, until we replaced all. In case a communication only has the sender and receiver as honest nodes, $\Pi_2$ and $\Pi_2^*$ are skipped for this communication, as the complete path was already replaced after $\Pi_1^*$.

$\boldsymbol{\Pi_2},\boldsymbol{\mathcal{A}_2}$: $\Pi_2$ behaves as $\Pi_1$, except that  for one communication the onion layers between a honest relay and the next honest node are replaced by other onion layers $O_i^R$. Those onion layers are the layers from an onion generated with random input in terms of message and path, except that the subpath between the current honest relay and the next honest node is part of the path.

\textbf{Indistinguishability 1 and 2:} As above ($0\rightarrow 1$), if there exists a distinguisher, it can be used to break $\OSNodeNode$.

$\boldsymbol{\Pi_2^*},\boldsymbol{\mathcal{A}_2^*}$: Replace onion layers on one subpath from honest relay to the next honest node (where they have not been replaced before) with random layers.

\textbf{Indistinguishability $\boldsymbol{2}$ and $\boldsymbol{2^*}$:} Analogous as above ($1\rightarrow 1^*$).\\

Finally, (in \(\Pi_3, \mathcal{A}_3\)) we replace the onion layers between the last honest relay and the corrupted receiver. The message is not chosen randomly as the adversary learns the message and could distinguish $\Pi_2^*$ from $\Pi_3$ otherwise.

$\boldsymbol{\Pi_3},\boldsymbol{\mathcal{A}_3}$: $\Pi_3$ behaves as $\Pi_2$, except that for one communication the onion layers that are output from the last honest relay are replaced with other onion layers. Those other layers $O_i^R$ are the ones of an onion that is created from a random input, except for the message and the last part of the path from the honest relay to the receiver. 


\textbf{Indistinguishability 2 and 3:} 
If there exists an distinguisher $\mathcal{D}$ that can distinguish outputs of $\Pi_2, \mathcal{A}_0$ from $\Pi_3, \mathcal{A}_0$, it can be used to construct an attack $\mathcal{A}$ on $\OSNodeReceiver$ analogous to the attack on $\OSSenderNode$ in the indistinguishability proof between 0 and 1.

%$\mathcal{A}$ uses the same communications as $\mathcal{A}_0$ for $b=0$ of $\OSNextNoHonest$\footnote{Analogous to above footnote.}. For $b=1$ the challenger picks the path before the honest node at random. $\mathcal{A}$ receives the first onions and the onions after each honest node from the challenger. $\mathcal{A}$ executes $\mathcal{A}_0$ except that it replaces the observing of onion layers with the onion layers received from the challenger (and uses procOnion on corrupted nodes, to generate the other onion layers that the challenger did not directly return, if needed). \todo[inline]{If $\mathcal{A}_0$ is an adaptive attack, $\mathcal{A}$ uses multiple challenges to allow for adaptivity.} The resulting outputs of $\mathcal{A}_0$ are given to the distinguisher $\mathcal{D}$, which returns a bit, that $\mathcal{A}$ uses as its guess $b'$.
%
%Clearly, in the scenario for $b=0$, the original onion layers are used and the execution of $\mathcal{A}_0$ equals the one with $\Pi_2$ being used; in the scenario for $b=1$ the subpaths after the honest nodes are replaced with random onions (including the same end of path and message), which equals the execution of $\mathcal{A}_0$ for $\Pi_3$. Hence, $\mathcal{A}$ does have the same success breaking $\OSNextNoHonest$ as the distinguisher $\mathcal{D}$ has distinguishing the protocols.\\

$\boldsymbol{\Pi_3^*},\boldsymbol{\mathcal{A}_3^*}$: Replace onion layers after the last honest relay to the corrupted receiver (where they have not been replaced before) with random layers.

\textbf{Indistinguishability 3 and $3^*$:} Analogous as above ($2\rightarrow 2^*$).\\

\paragraph*{Replacing with IDs} We now replace the random onion layers with IDs and in the case of corrupted receivers, random IDs and original messages. Each ID marks a subpath on which the adversary can link the onion layers. Since all other inputs are chosen randomly for the replacing onion layers, there is not less an adversary can learn from the IDs than before.\\
Attacks $A_4,A_5,A_6$ are done as before, except that instead of the onion layers now IDs are used (e.g. to drop, delay, modify) and the linking information (resp. the message) for the last subpath is deduced from the IDs (resp. attached in clear).

%Needs to be 4 from here on
$\boldsymbol{\Pi_4},\boldsymbol{\mathcal{A}_4}$: $\Pi_4$ behaves as $\Pi_3$, except that onion layers between honest nodes are replaced with random IDs. Each onion layer on the same subpath between honest node $P_i$ and next honest node $P_j$ is replaced by the same ID. The central storage used for ProcOnion is adapted accordingly.

$\mathcal{A}_4$ is done as $\mathcal{A}_3$ except that whenever the onion layers between honest nodes are used now the IDs are used and that when it does calculations to link those layers of the same onion now it only checks for them having the same ID. %Further, processOnion on such layers is adapted to return the ID and the next hop (that is saved in a list).\\

\textbf{Indistinguishability 3 and 4:}
From an onion layer an adversary can only learn something about the input to FormOnion.
As the onion layers are already randomly replaced at each honest node, linking onion layers before and after the honest node is not possible and nothing new about the input can be learned by processing the onion layers.
As the onion layers between honest nodes are already replaced by random onions that take the same path, $\mathcal{A}_3$ cannot learn more than the path between the honest nodes from those layers. Exactly the same can be learned from the IDs in $\mathcal{A}_4$ as it uses the adapted ProcOnion. 
Therefore, $\mathcal{A}_4$ simulates $\mathcal{A}_3$ and hence its outputs are indistinguishable from $\mathcal{A}_3$'s.\todo{that is not really a proper indistinguishability proof, its just argumentation.}

$\boldsymbol{\Pi_5},\boldsymbol{\mathcal{A}_5}$: $\Pi_5$ behaves as $\Pi_4$, except that any onion layer after the last honest node on the path is replaced with the same random ID and the included message.


$\mathcal{A}_5$ is done as $\mathcal{A}_4$ except that whenever the onion layers after the last honest node on the path are used now the IDs are used and that when it does calculations to link those layers of the same onion now it only checks for them having the same ID. Additionally, instead of doing procOnion multiple times to retrieve the message it uses the message that is part of the onion layer replacement. %Further, processOnion on such layers is adapted to return the ID  and message and the next hop (that is saved in a list).\\

\textbf{Indistinguishability 4 and 5:} 
Analogous to 3 and 4: Linking is prevented by the random replacement before. The information about the input to FormOnion that is accessible in $\mathcal{A}_4$ is also accessible for $\mathcal{A}_5$ as the subpath is clear in the IDs and the message attached and all other parts of the input were replaced by random choices before.\todo{same comment as above, no real proof}


$\boldsymbol{\Pi_6},\boldsymbol{\mathcal{A}_6}$: $\Pi_6$ behaves as $\Pi_5$, except that any onion layer where there is no honest node on the path (including sender and receiver) is replaced with the complete path, the message and the sender ID.

$\mathcal{A}_6$ is done as $\mathcal{A}_5$ except that whenever the onion layers of paths with no honest node are processed the information about the input is directly received without further calculations.

\textbf{Indistinguishability 5 and 6:} 
As the onion layers only depend on the input of FormOnion (and Randomness), this replacement allows $\mathcal{A}_6$ to learn all the inputs. As there is no honest node on the path, the same can be derived by using multiple processOnions. Hence, there is no more to learn from the onion layers as both $\mathcal{A}_5$ and $\mathcal{A}_6$ do. Therefore, $\mathcal{A}_6$ simulates $\mathcal{A}_5$ and hence its outputs are indistinguishable from $\mathcal{A}_5$'s.


$\boldsymbol{\mathcal{F}},\boldsymbol{\mathcal{S}}$: Ideal functionality $\mathcal{F}$ as described in Appendix \ref{app:idealFunctionality}.
Simulator $\mathcal{S}$ translates the outputs from $\mathcal{F}$ to  $\mathcal{A}_6$ and the actions of $\mathcal{A}_6$ to instructions for $\mathcal{F}$. We start with the passive observations.
When $\mathcal{S}$ gets the output that an ID (or an ID and a message) was sent along a subpath from $\mathcal{F}$, the simulator includes the ID as observation on the links between the relays and as observation of the corrupted relays along the path and gives it to $\mathcal{A}_6$.
By inspection of the descriptions for $\mathcal{A}_6$ and $\mathcal{S}$ their outputs are identical for an honest-but-curious adversary.

 Active parts of $\mathcal{A}_6$ are translated to actions in $\mathcal{F}$ by $\mathcal{S}$ as follows: Because of Assumption~\ref{ass:neglInfoOnInvalidInput}\todo{we might be able to weaken this assumption}, all active parts of attacks can be reduced to a combination of dropping and  inserting some onion layers\footnote{Notice that modification of an onion layer can be understood as dropping it and inserting the modified version.}. %that can be created as $ProcOnion^x(FormOnion(Input))$ (multiple processings of a created onion). 
 %Drop
 Dropping of an onion layer is done by never sending Deliver\_Message for this onion layer's ID for the next honest node on the path, if there is another honest node on the path.
 Further, in any case $\mathcal{S}$ does not forward the corresponding IDs (and messages) to $\mathcal{A}_6$ as observations of the corrupted relays or links after the relay that dropped the layer.
 %Insert
 Inserting of an onion layer $O_i$ is done by  $\mathcal{S}$ as follows: $S$ uses the knowledge of $\Pi_6$ to create an instance of the hybrid protocol and inserts the onion layer and observes the path it takes and the message it results in. Then it uses Process\_New\_Onion with this input in $\mathcal{F}$ and returns IDs (and message) as observations. In case that $O_i$ is a modification of an onion layer $O_i'$, $\mathcal{S}$ replaces the IDs (and message) from the outputs of $\mathcal{F}$ on the first following subpath with the $ID$ of $O_i'$\footnote{$\mathcal{S}$ can learn this IDs by stopping all other onions.}.
 Again, by inspection, the outputs for active attacks in$\mathcal{A}_6$ and $\mathcal{S}$ are identical.

The outputs of the ideal functionality and the machine that runs the protocol instances of \(\Pi_6\), that we introduced in the beginning, are identically chosen. \todo{enough?}%Again, by inspection, hybrid protocol \(\Pi_6\) works exactly as the ideal functionality $\mathcal{F}$.
As we translated any real world attack \(\mathcal{A}\) upon the secure onion routing protocol \(\Pi\) into a description for a simulator \(\mathcal{S}\) upon the protocol \(\Pi_6\), having shown that the output of \(\mathcal{A}\) and \(\mathcal{S}\) are indistinguishable and \(\Pi_6\) works identical to \(\mathcal{F}\), this concludes the proof.

\iflong
\textbf{Indistinguishability between view of \(\mathcal{A}_6\) of hybrid \(\Pi_6\) and \(\mathcal{S}\) of \(\mathcal{F}\):}
\todo[inline]{Do we still need to split cases for honest and dishonest receivers?}

\todo[inline]{I would remove this: We extend the definition of onion-correctness to also cover honest-but-curious adversaries that follow the protocol and do not actively drop, modify or insert new messages.}

Adversary \(\mathcal{A}_6\), as well as \(\mathcal{S}\) are allowed to statically select and compromise up to \(n-1\) mix nodes. % and choose their key pairs \((PK_i,SK_i)\).
Adversary \(\mathcal{A}_6\) and \(\mathcal{S}\) have access to \(\mathrm{FormOnion}_6, \mathrm{ProcOnion}_6(SK(P),\cdot,P)\), or \(Process\_New\_Onion, Deliver\_Message\) respectively.

The adapted \(\mathrm{ProcOnion}_6(SK(P),\cdot,P)\) of \(\Pi_6\), as well as \(Deliver\_Message\) of \(\mathcal{S}\) both accept an ID of an onion that should be processed by the next mix node.
If \(\mathcal{A}_6\) forwards an ID (uses \(\mathrm{ProcOnion}_6(SK(P),\mathrm{ID},P)\)) to a mix node \(P\) that is not the next mix node for the given ID, we have two possible cases:
If \(P\) is honest, it will get an incorrect onion and by our requirement that the protocol \(\Pi\) reveals only negligible information when an incorrectly generated onion is processed by an honest mix node, \(\mathcal{A}_6\) gains only negligible information.
If \(P\) is corrupted, there will be no gain as well, as \(\mathcal{A}_6\) already had the respective onion ID and all related information.

\(\mathrm{FormOnion}_6\), as well as \(Process\_New\_Onion\) accept a message \(m\), and a path of mix nodes \(\mathcal{P}\) and a receiver \(P_R\).

\(\mathrm{FormOnion}_6\) additionally accepts public keys for all nodes (incl. receiver), as well as a maximum path length.
As \(\mathcal{A}_6\) only receives random IDs, which are independent of the public keys given to \(\mathrm{FormOnion}_6\), the choice of public keys does not help distinguishing the view of \(\mathcal{A}_6\) from \(\mathcal{S}\).
The maximum path length is a system parameter.
If \(\mathcal{A}_6\) uses an incorrect maximum path length as input to \(\mathrm{FormOnion}_6\), honest routers will not be able to process the created onion correctly and by our requirement that the protocol \(\Pi\) reveals only negligible information when an incorrectly generated onion is processed by an honest mix node, selecting a maximum path length that differs from the system parameter does not help in distinguishing the view of \(\mathcal{A}_6\) from \(\mathcal{S}\).

\(Process\_New\_Onion\) additionally accepts as input next to the actual path, the length of the path \(n\). However, in \(\mathcal{F}_{Onion}\) the path length given to \(Process\_New\_Onion\) must be correct: \(n = |\mathcal{P}|\).
As \(\mathrm{FormOnion}_6\) can trivially determine \(n\), and \(\mathcal{S}\) must input the correct \(n\), there is no additional information carried in this parameter, which could help distinguishing the view of \(\mathcal{A}_6\) from \(\mathcal{S}\).

Given adversaries \(\mathcal{A}\) and \(\mathcal{S}\) created an onion using \(\mathrm{FormOnion}_6\) (\(Process\_New\_Onion\), respectively) they both receive a random ID representing the created onion.
As they created the onion, both adversaries know the path of mix nodes, the path length, the sender and the receiver belonging to the received ID.
Both adversaries also receive a random and independently chosen session ID \(sid\) belonging to that onion.

If an onion should be sent from node \(P_{i}\) to \(P_{i+1}\) both adversaries learn the current random onion ID, as well as the sending node identifier \(P_i\).
If node \(P_{i+1}\) is honest, they both also learn \(P_{i+1}\) and nothing else.
If \(P_{i+1}\) is corrupted, they additionally learn the path of corrupted nodes \((P_{i+1},\ldots,P_j)\) including the next honest node \(P_j\).
In \(\Pi_6\) this is true as the temporary ID for an onion is not changed over a sequence of consecutive corrupted nodes.
If there is no honest node remaining, the learned path includes the receiver \((P_{i+1},\ldots,P_R)\) and (as the receiver is corrupted ($\OSVeryStrong$)\todo{check symbol}) the actual massage \(m\).

If in such an onion forwarding scenario the sender of the original onion was corrupted, both adversaries further receive (also if the next hop is honest) the respective session id \(sid\), through which they can link the current temporary onion ID to the original onion with the belonging sender \(P_S\), receiver \(P_R\), message \(m\) and path \(\mathcal{P}\).

Before any such forwarding of onions to the next mix node actually happens, the adversaries must allow their forwarding.
\(\mathcal{A}_6\) does this by not dropping the received ID and actually forwarding it to the next mix node.
\(\mathcal{S}\) calls \(Deliver\_Message\) using the temporary ID for the onion that should be forwarded. \\

\textbf{Case 2: Honest Receiver (\(\OSVeryVeryStrong\)\todo{check symbol}):} \\

%Hybrid protocol $\boldsymbol{\Pi_0'}$ and habrid adversary $\boldsymbol{\mathcal{A}_0'}$ are identical to the first case.
%Following hybrid protocols $\boldsymbol{\Pi_1},\boldsymbol{\Pi_2},\boldsymbol{\Pi_4}$ and hybrid adversaries $\boldsymbol{\mathcal{A}_1},\boldsymbol{\mathcal{A}_2},\boldsymbol{\mathcal{A}_4}$ are similar to case 1, except for construction of attacks on \(\OSVeryVeryStrong\) instead of \(\OSVeryStrong\).

The indistinguishability of views \(\mathcal{A}_6\) of hybrid \(\Pi_6\) and \(\mathcal{S}\) of \(\mathcal{F}_{Onion}\) again is similar, except for the following situation in which an onion should be sent from node \(P_{i}\) to \(P_{i+1}\) and \(P_{i+1}\) is corrupted:
If there is no honest node remaining, the learned path includes the receiver \((P_{i+1},\ldots,P_R)\), but \emph{not} the actual massage (as the receiver is \emph{not} corrupted ($\OSVeryVeryStrong$).


\todo[inline]{Some notes follow and might be removed later on}

\todo[inline]{Completely strange late evening thought: I can translate any attack to the dropping all but 1 attack, in which I learn the complete path and (if corrupted receiver) the message. Hence, in this case I must learn at least as much as in the original attack. Thus, any protocol (with correct encryption, as the receiver needs to be corrupted to learn the message) realizes this ideal functionality. In other words: this concept of splitting the adversary and not looking at timing attacks/dropping might not really go well with UC? Is there a way to fix this?}

\todo[inline]{check all ideal functionality/protocol uses; there is a difference between ideal protocol and ideal functionality} 
\fi

\iflong
\todo[inline]{following unclear if needed anymore...}
\subsubsection{Observations regarding privacy attacks on onion routing}

\paragraph{Goals}
\begin{itemize}
	\item reduce anonymity set size (can be done arbitrarily in ideal functionality by dropping messages)
	\item learn new information:
	\begin{itemize}
		\item Randomness, Keys (Protected by Assumption \ref{})
		\item Input to $\mathrm{FormOnion}$:
			\begin{itemize}
				\item path, path length
				\item message, message length
				\item auxiliary information 
				\begin{itemize}
					\item  $aux_1$ (needs to be protected and part of the properties)
					\item  $aux_2$ (not protected, hence no need to deal with; like forward/backward bit)
					\item  maybe randomness (can be  simulated in FormOn, with the protected randomness) and things derived from protected keys (same as randomness..))
				\end{itemize}
			\end{itemize}
	\end{itemize}
\end{itemize}
\todo[inline]{Move goals to properties imply functionality proof?}

\paragraph{Attacks possible on Ideal functionality}
\begin{itemize}
	\item Dropping, Delaying, Replacing Onion (with results from FormOnion), Inserting (results from FormOnion)
\end{itemize}

\paragraph{Remaining Attack possibilities}
\begin{itemize}
	\item learn something one onion from the onion itself, i.e. their processed layers; maybe modified (we will make sure this does not happen by replacing the onion layers with layers from other random `fake' onions without the adversary noticing it)
	\item learn something about one onion because of its relation to other onions (existing really in the network), i.e. being able to distinguish the observed onion from other `real' onions after it passed honest relays (we will make sure this cannot happen by a property that allows the adversary to modify the observed one and where she has to distinguish it from another one \todo{rewrite later}) 
\end{itemize}
\fi




==> sections/unused/proofImplyIdealDuplicates.tex <==
\label{app:proofImplyIdealMod}

The simulator works as before.
The argument uses the same machines, but needs to differ in one indistinguishability step. 

$\mathbf{\mathcal{H}_0\approx_I \mathcal{H}_1^1}$. 
The adversary observes the onion layers after the honest sender $P_0$ and  if it gives an onion to the honest node $P_j$ the result of the processing after the honest node. Depending on the behavior of $\mathcal{A}$ three things can happen, the onion is belonging to this communication is dropped before $P_j$, the adversary behaves protocol-conform and sends the expected onion to $P_j$ or the adversary modifies the expected onion with some modification function\footnote{Any modification to an earlier onion layer than the one directly before $P_j$ can be translated into a modification of the onion layer directly before $P_j$.} $f$ before sending it to $P_j$.
 
 Notice that not modifying the expected onion is a special version of the last case where $f$ is the identity function $id$ and that dropping the onion only leaves the adversary with less output on which the cases can be distinguished. Hence if the case of more outputs cannot be distinguish, neither the case with less outputs can. Thus we can focus on the case with the modification function $f$, that might or might not be $id$.
 
 We assume there exists an distinguisher $\mathcal{D}$ between $\mathcal{H}_0$ and $\mathcal{H}_1^1$. Depending on whether $f$ behaves like $id$ on the chosen onions $O_j$ and $\bar{O}_j$ we can construct a successful attack on another onion property\footnote{Even if $f$ behaves non-deterministic on the onions, one of the cases occurs with non-negligible probability and in each we win again with non-negligible advantage.}.
 
 Case a: $f(O_j)=O_j$ and $f(\bar{O}_j)=\bar{O}_j$: We construct an attack on $\OSSenderNode$. 
 The attack receives key and name of the honest relay and uses the input of the replaced communication as choice for the challenge, where it replaces the name of the first honest relay with the one that it got from the challenger\footnote{As both honest nodes are randomly drawn this does not change the success}\todo{Do I need an assumption that the name does not influence what the adv learns?}. For the other relays the attack decides on the keys as $\mathcal{A}$ (for corrupted) and the protocol (for honest) does. It receives an onion $(\tilde{O}, \ProcOnion{O_j})$ from the challenger. The attack uses $\mathcal{D}$. For $\mathcal{D}$ it simulates all communications except the one chosen for the challenge with the oracles and knowledge of the protocol and keys. For simulating the challenge communication the attack hands $\tilde{O}$ to $\mathcal{A}$ as soon as $\mathcal{D}$ instructs to do so and on behalf of further simulating for $\mathcal{D}$ uses $\tilde{O}$ to calculate the further layers, does any actions $\mathcal{A}$ does on the onion and if the honest-processing of $\tilde{O}$ is send from the adversary to the honest challenge router $\ProcOnion{O_j}$ is given to $\mathcal{A}$. Thus, in the result either the challenger chose $b=0$ then the attack behaves like $\mathcal{H}_0$ under the distinguisher $\mathcal{D}$; or the challenger chose $b=1$ then the attack behaves like $\mathcal{H}_1^1$ under the distinguisher $\mathcal{D}$. The attack thus only needs to output the same bit as $\mathcal{D}$ does for its simulation to win with the same advantage as $\mathcal{D}$ can distinguish the hybrids.
 
 Case b: $f(O_j)\neq O_j$ and $f(\bar{O}_j)\neq \bar{O}_j$: We construct an attack on $\OSMod$ similar to Case a: We use the same choice for the challenge and additionally pick $f$ as $\mathcal{A}$ modifies onions. Notice that similar to $\OSSenderNode$ in case a, the attack uses the two onions output by the $\OSMod$ challenger when communicating with the adversary $\mathcal{A}$ as $\mathcal{D}$ prescribes. Thus, if $b=0$ in the $\OSMod$ game the attack creates the same behavior as $\mathcal{H}_0$ and $b=1$ as $\mathcal{H}_1^1$ and again the guess of distinguisher $\mathcal{D}$ is chosen as the output to achieve the same advantage.
 
 Case c: ($f(O_j)= O_j$ and $f(\bar{O}_j)\neq \bar{O}_j$) or $f(O_j)\neq O_j$ and $f(\bar{O}_j)= \bar{O}_j$:
 We can construct one of the above attacks as both of the cases that one returns the output as $id$ need to happen with a similar probability as we show now:
 Assume there exists a modification $f$ such that \(Pr[f(O_j)=O_j \mid  O_j\text{ chosen as layer of }\FormOnion(\text{Adversary Input})] - Pr[f(\bar{O}_j)=\bar{O}_j \mid  \bar{O}_j\text{ chosen as the replacement layer above}] \geq \delta \) with $\delta$ non negligible. Based on this we can construct a successful attack on $\OSSenderNode$: $\mathcal{A}_{\OSSenderNode}$ uses the same input for the challenge communication and receives $(O,O')$ from the challenger. If $f(O)=O$ $\mathcal{A}_{\OSSenderNode}$ guesses 0. Otherwise, 1. The success of this attack is 
 \[\frac{1}{2}Pr[g=0\mid b=0]+\frac{1}{2}Pr[g=1\mid b=1]=\]
 \[\frac{1}{2}Pr[f(O_j)=O_j]+\frac{1}{2}Pr[f(\bar{O}_j\neq \bar{O}_j]>\frac{1}{2}+\frac{1}{2} \delta\text{.}\] 
 
 Thus, we can assume that the probability of the modification behaving like $id$ is nearly equal for both onions. Hence, if this probability is non negligible for $O_j$ the attack of case a works with non negligible probability. Otherwise, the attack of case b works with non negligible probability. So with non negligible probability one of the attacks has non negligible advantage, which means the corresponding onion property is not fulfilled. 
 



==> sections/wrapResistance.tex <==
We describe a template for adding wrap-resistance of~\cite{camenisch2005formal} (see Appendix \ref{app:originalDef}) to any \ac{OR} protocol without changing what the adversary can learn. % that sends a message over at least one intermediate hop.
%We proof wrap-resistance and show that the output of the original protocol and the adapted protocol are indistinguishable for a (n-2) adversary (sender and one intermediate hop are honest).\todo{for what is the intermediate hop needed?}
It follows that the wrap-resistance property is not related to any privacy goal in anonymous communication.
We show our results for an \ac{OR} protocol, but the result applies in general; also for other protocols.


\paragraph{Protocol Extension}\label{sec:wrapResistantProtocol}
We assume that the intermediate routers running the \(\mathrm{ProcOnion}\) algorithm have local storage to keep a persistent counter next to their secret key.\footnote{Otherwise, this counter could also be securely (achieving confidentiality, integrity and freshness) stored and retrieved on another server.}
We use a secure key derivation function (KDF) to generate ephemeral keys at intermediate routers.
We make use of a secure, symmetric MAC system, which generates tags that are indistinguishable from random values for any \ac{PPT} adversary.
That is, we require the signing function \(t = \mathrm{sign}(k,m)\) operating over a key \(k\), a message \(m\) and generating a tag \(t \) within tag space \(\mathcal{T}\)  to be a pseudo-random function (PRF)\footnote{ Such a signing function exists:
HMAC is a PRF, if the underlying compression function is a PRF~\cite{bellare_new_2006} .
In the random oracle model, cryptographic hash functions (can be used as compression functions) are treated as random functions.
Thus, using HMAC with a cryptographic hash function as compression function fulfills our requirement in the random oracle model.}.


Let \(\Pi\) be an \ac{OR} protocol that transfers a message \(m\) from a sender \(P_0\) to a receiver \(P_{n+1}\) over \(n\) intermediate routers \(\{P_i\}\) for \(1 \leq i \leq n\).
Here is how to create the extended protocol \(\Pi_{wr}\) using \(\mathrm{FormOnion}_{wr}\) and \(\mathrm{ProcOnion}_{wr}\).

\paragraph*{Sender [\(\mathrm{FormOnion}_{wr}\)]}
The sender runs the original algorithm  \(\mathrm{FormOnion}\) as specified by \(\Pi\). Additionally, for any packet $p$ that the protocol sends from the sender to the first intermediate router, it appends a random number  \(r_0 \in \mathcal{T}\) of the tag space created using a secure pseudo random number generator. The resulting onion \(p'_1 = p_1|r_0\) is sent to \(P_1\).
%
%The sender runs the original algorithm \(\mathrm{FormOnion}\) as specified by \(\Pi\). Additionally, for any packet \(p\) that the protocol sends from the sender to the first intermediate router the following steps are performed. Let \(|\) denote concatenation.
%\begin{enumerate}
%  \item[\(P_S\)] generates a random number \(r_s\) using a secure pseudo random number generator.
%    The random number \(r_s \in \mathcal{T}\) is chosen out of the tag space of the MAC system.
%  \item[\(P_S\)] sends the packet \(p'_1 = p_1|r_s\) to the first intermediate router \(P_1\).
%\end{enumerate}

\paragraph*{Intermediate Router [ \(\mathrm{ProcOnion}_{wr}\)]}
Any intermediate router receiving a packet \(p'_i=p_i|t_{i-1}\)  removes and stores the received tag \(t_{i-1}\) (or random number \(t_{i-1}=r_s\) if it is the first intermediate router) to retrieve the original packet \(p_i\). Then it runs \(\mathrm{ProcOnion}\) as by the protocol \(\Pi\)  on \(p_i\) to create \(p\). Afterwards it uses the KDF function to derive an ephemeral key \(k_i = \mathrm{KDF}(SK_i,s)\) from its own secret key \(SK_i\) and the internal state \(s \in \mathbb{N}\), increases the internal state by one \(s \gets s + 1\) and generates a tag \(t_i = \mathrm{sign}(k_i,P_i)\) using the secure MAC signing function with key \(k_i\) upon the identity \(P_i\). Finally, it sends  the packet \(p' = p|t_i\)  to the next hop \(P_{i+1}\)

%
%\paragraph*{Receiving at intermediate router}[Desciption of first part of \(\mathrm{ProcOnion}_{wr}\)]
%Any intermediate router receiving a packet \(p'_i\) performs the following steps before running \(\mathrm{ProcOnion}\) as by the protocol \(\Pi\) for a received packet \(p'_i = p_i|t_{i-1}\).
%\begin{enumerate}
%  \item[\(P_i\)] removes the received tag \(t_{i-1}\) (or random number \(r_s\) if it is the first intermediate router)
%  \item[\(P_i\)] retrieves the original packet \(p_i\).
%\end{enumerate}
%After these steps, \(P_i\) operates on \(p_i\) using \(\mathrm{ProcOnion}\) as the original protocol \(\Pi\) requires.
%
%\paragraph*{Sending at intermediate router}[Desciption of last part of \(\mathrm{ProcOnion}_{wr}\)]
%After running \(\mathrm{ProcOnion}\) as by the protocol \(\Pi\) and before sending any packet \(p_{i+1}\) it performs the following steps.
%\begin{enumerate}
%  \item[\(P_i\)] uses the KDF function to derive an ephemeral key \(k_i = \mathrm{KDF}(SK_i,s)\) from its own secret key \(SK_i\) and the internal state \(s \in \mathbb{N}\).
%  \item[\(P_i\)] increase the internal state by one \(s \leftarrow s + 1\)
%  \item[\(P_i\)] generates a tag \(t_i = \mathrm{sign}(k_i,P_i)\) using the secure MAC signing function with key \(k_i\) upon the identity \(P_i\).
%  \item[\(P_i\)] sends the packet \(p' = p|t_i\) either to the next intermediate router \(P_{i+1}\) or in case \(i=n\) to the receiver \(P_R\).
%\end{enumerate}

\paragraph*{Receiver}[Identical to first part of \(\mathrm{ProcOnion}_{wr}\)]
The receiver getting the packet \(p'_{n+1}=p_{n+1}|t_n\) removes the tag \(t_{n}\), retrieves the original packet \(p_{n+1}\) and operates on it as by the original protocol description.

\paragraph{Analysis}

Let the wrap-resistance game be defined as given by Camenisch where it is part of ``onion-security''. The extracted game (Definition~\ref{def:wrapResistance}) can be found in Appendix~\ref{app:originalDef}.

\begin{theorem}\label{thm:wrapResistance}
  The extended protocol \(\Pi_{wr}\) as described above achieves wrap-resistance.
\end{theorem}

  We prove this theorem by contradiction.
  We assume that we can break wrap resistance given the extended protocol and reduce it to finding a collision for a cryptographically secure MAC system (thus breaking the MAC).

\begin{proof}
  Assume that the extended protocol \(\Pi_{wr}\) does not achieve wrap-resistance as given by Definition~\ref{def:wrapResistance}.
  As the adversary can break wrap resistance, there exists an identity \(P' \neq P_{j-1}\) for which she can efficiently generate \(SK',O'\) such that \((P'', O_j) = \mathrm{ProcOnion}_{wr}(SK',O',P')\).
  That is, she can efficiently generate a second pre-image on \(\mathrm{ProcOnion}_{wr}\) to generate a collision on the onion output \(O_j\) under different identities \(P_{j-1} \neq P'\).
  Based on this efficient algorithm, we can construct an efficient algorithm that generates a collision by finding a second pre-image on the signing function of the underlying secure MAC system, which adds a tag to any onion.
  This contradicts the assumption of the secure MAC system.
\end{proof}

It remains to show that our extension is not changing the information an adversary can learn.
\todo[inline]{DOES NOT HAVE OS... is still a problem here: if techniques to extend $\Pi$ are limited to the ones that keep OS, those might always add to the privacy, hence we cannot really say that wrap-resistance is useless..
Solution idea: as above shared symm key between sender and relay, sender precomputes tags and sends them encrypted (however, if sender keeps and sends state,  adv could learn e.g. how many msgs sender send in total (which could be more than possible before if original protocol has some cover traffic...)so pick state random.)}
 
\begin{theorem}[Adversary learns the same information]\label{thm:learnsSame}
  Given extended protocol \(\Pi_{wr}\) as described above, an adversary learns the same information as running the original protocol \(\Pi\).
\end{theorem}
  
%\begin{theorem}[Adversary learns not less]\label{thm:learnsNotLess}
%  Given a an extended protocol \(\Pi_{wr}\) as described above, an adversary learns at least as much information as running the original protocol without the extension.
%\end{theorem}
\begin{proof}We show that an adversary neither learns less, nor more.
\setcounter{paragraph}{0}
\emph{a) Learns not less}
  %The original protocol is wrapped by some steps before sending a packet and after receiving one for all participating parties.
  In protocol \(\Pi_{wr}\) any router receives a packet \(p'=p|t_i\), which includes \(p\), i.e. the packet the same router would receive in \(\Pi\). Thus, it learns all the information it would learn in \(\Pi\).
%  In both cases it learns \(p\) and operates on it using \(\mathrm{ProcOnion}\), which is part of \(\mathrm{ProcOnion}_{wr}\) in \(\Pi_{wr}\).
%  Thus in the extended protocol \(\Pi_{wr}\), the adversarial router learns at least as much as he would running the original protocol.
%  The same argumentation holds for an adversarial receiver.
  %The receiver also gets \(p\), either directly (\(\Pi\)), or as part of \(p'\) (\(\Pi_{wr}\)).
  
  \emph{b) Learns not more}
  We prove this using two steps. First we extend the original protocol \(\Pi\) another way using fresh random numbers at any sending step (creating protocol \(\Pi_r\)) and show that adding fresh random numbers to any packet does not give an adversary any information. Then in a second step we compare \(\Pi_r\) to the extended wrap-resistant protocol \(\Pi_{wr}\) and show indistinguishability between them.
  
  \todo{Rest in App?}
    \emph{Randomized \ac{OR} protocol (\(\Pi_r\)):}
  For any packet \(p\) that is being sent by either the sender or any intermediate router, a fresh random number \(r\) is generated and appended to the packet \(p\).
  The random value \(r\) is chosen independently and uniformly at random out of the tag space of the secure MAC system.

  \emph{No information gain by random values (\(\Pi \rightarrow \Pi_r\)):}
  The length of the random value is a publicly known system parameter and carries no information for the adversary.
  Clearly, appending an independently chosen random value to a packet does not transfer any information to an honest-but-curious adversary.
  Malicious adversaries can send arbitrary content, however, as any honest router discards the appended data, there is no way to carry information over an honest router using the appended data.
  As such, the extra data in \(\Pi_r\) does not give the adversary any information gain over the plain packet without extra data as given by \(\Pi\).

%  \todo[inline]{rewrite using a game. Challenger plays either \(\Pi_r\) or \(\Pi_{wr}\).}
  \emph*{Indistinguishability of randomized and wrap-resistant protocol (\(\Pi_r \rightarrow \Pi_{wr}\)):}
  As the beginning of the packets in \(\Pi\) and \(\Pi_{wr}\) are identical, the adversary cannot not use them to distinguish \(\Pi_r\) from \(\Pi_{wr}\).
  
  Packets either stem from the sender or an intermediate router:
  \emph{Case 1 (packet \(p\) from sender):}
  As the pseudo-random value \(r_s\) appended by \(\Pi_{wr}\) has the same length as \(r\) appended by \(\Pi_r\), the length cannot be used to distinguish the protocols.
  Further, as \(r_s \in \mathcal{T}\) is chosen by a secure PRNG, they are indistinguishable from random values by a \ac{PPT} adversary.
  Thus the adversary cannot distinguish the protocols by packets coming from the sender.

  \emph{Case 2 (packet \(p\) from intermediate router):}
  As the value \(t_i\) appended by \(\Pi_{wr}\) has the same length as \(r\) appended by \(\Pi_r\), the length cannot be used to distinguish the protocols.
  A secure MAC generating pseudo-random tags is used to generate \(t_i\), thus it is indistinguishable from random values.
  
\end{proof}

%\begin{theorem}[Adversary learns not more]\label{thm:learnsNotMore}
%  Given an extended protocol as described above, an adversary learns not more information than running the original protocol without the extension.
%\end{theorem}

%\begin{proof}
%  First we describe another extension that appends fresh random values for all sent packets.
%
%  \paragraph*{Randomized \ac{OR} protocol (\(\Pi_r\))}
%  For any packet \(p\) that is being sent by either the sender or any intermediate router, a fresh random number \(r\) is generated and appended to the packet \(p\).
%  The random value \(r\) is chosen independently and uniformly at random out of the tag space of the secure MAC system.
%
%  \paragraph*{No information gain by random values (\(\Pi \rightarrow \Pi_r\))}
%  The length of the random value is a publicly known system parameter and carries no information for the adversary.
%  Clearly, appending an independently chosen random value to a packet does not transfer any information to an honest-but-curious adversary.
%  Malicious adversaries can send arbitrary content, however, as any honest router discards the appended data, there is no way to carry information over an honest router using the appended data.
%  As such, the extra data in \(\Pi_r\) does not give the adversary any information gain over the plain packet without extra data as given by \(\Pi\).
%
%%  \todo[inline]{rewrite using a game. Challenger plays either \(\Pi_r\) or \(\Pi_{wr}\).}
%  \paragraph*{Indistinguishability of randomized and wrap-resistant protocol (\(\Pi_r \rightarrow \Pi_{wr}\))}
%  As the beginning of the packets in \(\Pi\) and \(\Pi_{wr}\) are identical, the adversary cannot not use them to distinguish \(\Pi_r\) from \(\Pi_{wr}\).
%
%\begin{itemize}
%  \item{Case 1 (packet \(p\) from sender):}
%  As the pseudo-random value \(r_s\) appended by \(\Pi_{wr}\) has the same length as \(r\) appended by \(\Pi_r\), the length cannot be used to distinguish the protocols.
%  Further, as \(r_s \in \mathcal{T}\) is chosen by a secure PRNG, they are indistinguishable from random values by a polynomial time adversary.
%  Thus the adversary cannot distinguish the protocols by packets coming from the sender.
%
%  \item{Case 2 (packet \(p\) from intermediate router):}
%  As the value \(t_i\) appended by \(\Pi_{wr}\) has the same length as \(r\) appended by \(\Pi_r\), the length cannot be used to distinguish the protocols.
%  A secure MAC generating pseudo-random tags is used to generate \(t_i\), thus it is indistinguishable from random values.
%  \end{itemize}
%\end{proof}

